Improved Regret for Differentially Private Exploration in Linear MDP

We study privacy-preserving exploration in sequential decision-making for environments that rely on sensitive data such as medical records. In particular, we focus on solving the problem of reinforcement learning (RL) subject to the constraint of (joint) differential privacy in the linear MDP setting, where both dynamics and rewards are given by linear functions. Prior work on this problem due to Luyo et al. (2021) achieves a regret rate that has a dependence of $O(K^{3/5})$ on the number of episodes $K$. We provide a private algorithm with an improved regret rate with an optimal dependence of $O(\sqrt{K})$ on the number of episodes. The key recipe for our stronger regret guarantee is the adaptivity in the policy update schedule, in which an update only occurs when sufficient changes in the data are detected. As a result, our algorithm benefits from low switching cost and only performs $O(\log(K))$ updates, which greatly reduces the amount of privacy noise. Finally, in the most prevalent privacy regimes where the privacy parameter $\epsilon$ is a constant, our algorithm incurs negligible privacy cost -- in comparison with the existing non-private regret bounds, the additional regret due to privacy appears in lower-order terms.

==> files/DP_update_lemma.tex <==
{\color{blue}NOTE: Try proving with lemma from \cite{gao2021provably}. I think we cannot use this proof for the private case. The reason is that this proof requires a potential argument, and for that they need to bound the potential function by $O(d\log(T))$. but with privacy the potential function they use will depend on $\eps$. }

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Lemma: Bounding updates
%% Make Lemma general enough that it can be applied to the linear bandits setting.
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{lem:DPSwitchingcost}
Let $\phibf_1, \ldots, \phibf_T$ be a  sequence  of length $T$, where each $\phibf_t\in\bbR^d$ is a $d$-dimensional vector and for all $t\in[T]$ it holds that $\nn{\phibf_t}_2\leq 1$. 
%
For each $0<t\leq T$, define $\W_t = \sum_{i=1}^{t} \phibf_i \phibf_i^\top + \V$
and $\Wtil_t = \W_t + \mH_t$.
The matrix $\V\in \bbR^{d\times d}$  is a positive semidefinite matrix with $\V \succ \mH_t $ for all $0< t \leq T$. 
Note that $\Wtil_0 = \W_0 = \V$.
Let $c>1$ be any constant and say that there is a trigger event on time $t$ if $\det\pp{\Wtil_t} \geq c \det\pp{\Wtil_{\tau}}$, where $\tau<t$ is the time of the last trigger event before $t$ or 0 if $t$ is the first trigger event.

If there exists $\lambda>0$ such that $\mathrm{tr}(\V) \leq  d\lambda$, $\det\pp{\V} \geq \lambda^d$ and $d\lambda \geq \frac{T}{T-1} $, then the number of trigger events is at most $d  \LOG{c}{T}$.
\end{lemma}
% \begin{remark}
% We can satisfy the assumption in \cref{lem:Switchingcost} by setting $\V = \lambda \I$. 
% Note that to set the right value of $\lambda$ we must know $T$ in advance.
% \end{remark}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
\newcommand{\ki}[1]{k_{[#1]}}


Let $K$ be the total number of trigger events at the end of  $T$ rounds and let $\ki{0}, \ldots, \ki{K}$ be the trigger event times. By definition the first and last rounds are trigger events, thus we have $\ki{K} = T$  and $\ki{0} = 0$. We proceed by assuming that $K > d\LOG{c}{T}$ and show that this leads to a contradiction.

First, by definition of a trigger event on time $\ki{K}$ we have 
%
\begin{align}\label{eq:mainI}
    c \DET{\Wtil_{\ki{K-1}}} \leq \DET{\Wtil_{\ki{K}}}
\end{align}

If we unfold the recursion given by \cref{eq:mainI} and starting with $c \DET{\Wtil_{\ki{K-1}}} $ we get the following inequality
\begin{align}\label{eq:inductiveinequalityI}
    c\DET{\Wtil_{\ki{K-1}}}
    \geq c^2 \DET{\Wtil_{\ki{K-2}}}
    \geq c^3 \DET{\Wtil_{\ki{K-3}}}
    \geq \ldots 
    \geq c^{K} \DET{\Wtil_{\ki{0}} }
\end{align}

Note that $c^{d\LOG{c}{\ki{K}}}  = c^{\LOG{c}{\ki{K}^d}}  = \ki{K}^{d}$.
Since $c>1$ and by the assumption that $K > d\LOG{c}{\ki{K}}$, the following holds $c^{K} > c^{d\LOG{c}{\ki{K}}}=\ki{K}^{d}$. Therefore, combining \cref{eq:mainI} and \cref{eq:inductiveinequalityI} and replacing $K$ with $ d\LOG{c}{\ki{K}}$ we have
%
\begin{align}
\label{eq:mainII}
    \text{\cref{eq:mainI}, \cref{eq:inductiveinequalityI}} \text{ and } K > d\LOG{c}{\ki{K}}
    \implies \ki{K}^{d} \DET{\Wtil_{\ki{0}} } < \DET{\Wtil_{\ki{K}}} 
\end{align}
%
Next, we use the fact that the determinant a matrix is equal to the product of its eigenvalues and the trace of a matrix equals the sum of its eigenvalues and we use the  inequality of arithmetic and geometric means to get
%
\begin{align}\label{eq:AGmeans}
    \DET{\Wtil_{\ki{K}}} \leq \pp{\frac{\text{tr}\pp{\Wtil_{\ki{K}}}}{d}}^d 
    % \label{eq:clogD}
    % c^{d\LOG{c}{\ki{K}}}  = c^{\LOG{c}{\ki{K}^d}}  = \ki{K}^{d}
\end{align}

Combining \cref{eq:mainII}, \cref{eq:AGmeans} we get
%
\begin{align} \label{eq:mainIII}
    \text{\cref{eq:mainII}, \cref{eq:AGmeans}} \implies 
    \ki{K}^{d}\DET{\Wtil_{\ki{0}} } < \pp{\frac{\text{tr}\pp{\Wtil_{\ki{K}}}}{d}}^d
\end{align}

For the next step, we use the  fact that $\text{tr}\pp{\W_{\ki{K}}} \leq \text{tr}\pp{\W_{0}} + \ki{K} $, which follows from the assumption that $\nn{\phibf_i}_2^2 \leq 1$. Also for any $t$, since $\W_0 \succ \mH_t$ we have that $\text{tr}\pp{\W_{0}} \geq  \text{tr}\pp{\mH_{t}}$. Then we get the following inequality

\begin{align}
 \label{eq:mainIIIandI}
    \text{tr}\pp{\Wtil_{\ki{K}}}  &= \text{tr}\pp{\W_{\ki{K}}} +  \text{tr}\pp{\mH_{\ki{K}}} \leq \text{tr}\pp{\W_{0}} + \ki{K}+ \text{tr}\pp{\mH_{\ki{K}}}
    \leq  2\text{tr}\pp{\W_{0}} + \ki{K}
\end{align}

Then it follow from \cref{eq:mainIII}, \cref{eq:mainIIIandI} that

\begin{align} 
\notag
    \text{\cref{eq:mainIII}, \cref{eq:mainIIIandI}} &\implies 
    \ki{K}^{d}\DET{\Wtil_{\ki{0}} } < \pp{\frac{2\text{tr}\pp{\W_{\ki{0}}}  + \ki{K}}{d}}^d \\ 
\label{eq:mainIV}
    &\implies \ki{K}^{d}\DET{\V} < \pp{\frac{2\text{tr}\pp{\V}  + \ki{K}}{d}}^d && \pp{\text{Recall }\W_{\ki{0}} = \Wtil_{\ki{0}} = \V} 
\end{align}

Dividing $\ki{K}$ on both sides of equation \cref{eq:mainIV} we get
\begin{align} \label{eq:mainV}
    \DET{\V} 
    <  \pp{\frac{2\text{tr}\pp{\V}  + \ki{K}}{d \ki{K}}}^d  
    = 
    \pp{\frac{2\text{tr}\pp{\V}}{d \ki{K}} 
    + \frac{1}{d}
    }^d
\end{align}

We assumed that $\DET{\V} \geq \lambda^d$ and that $\text{tr}\pp{\V} \leq d\lambda$, thus \cref{eq:mainV} implies
\begin{align} 
\notag
\text{\cref{eq:mainV}} &\implies 
    \lambda^d < \pp{\frac{2d\lambda}{d \ki{K}} + \frac{1}{d} }^d  \\
    \label{eq:mainVI}
    &\implies
    1 <  \pp{\frac{2d\lambda}{d \lambda\ki{K}} + \frac{1}{d\lambda} }^d 
    =  \pp{\frac{2}{\ki{K}} + \frac{1}{d\lambda} }^d 
    = \pp{\frac{2}{T} + \frac{1}{d\lambda} }^d && \pp{\text{Since } \ki{K} = T}
\end{align}

Since we choose $d\lambda $ s.t $\frac{2}{T} + \frac{1}{d\lambda} \leq 1$ then \cref{eq:mainVI} is a contradiction completing the proof.
\end{proof}



==> files/LinearMAB/analysis.tex <==
% \section{Analysis of \cref{alg:slowlinearbandits}}
%
% \input{files/DP_update_lemma}

% This section focuses on the linear bandits problem. First we describe the problem setting: 
% On each round $t\in[T]$, a learner observes a finite decision set $\cX_t\subset \mathbb{R}^d$ and chooses an action $\x_t\in \cX_t$. 
% Then the learner observes a reward $y_t$, which is given by 
% \begin{align*}
%     y_t = \vdot{\thetabf^*, \x_t} + \etabf_t
% \end{align*}
% where $\thetabf^*$ is called the true parameter vector and $\etabf_t$ is noise term.



% For privacy we shift the Gram matrix by the Gaussian noise matrix to get the private Gram matrix $\Vtil_t := \V_t + \Z_t$. We also have $\lambda \in \mathbb{R}$ such that with high probability we have $\Vtil_t + \lambda \I \succ 0$ is positive semidefinite  and for all $t\in [T]$.


% \begin{lemmarep} 
% \cite{Paksoy2014INEQUALITIESOG}
% Let $\A, \textbf{B}$ be positive semidefinite matrices of equal size. Then
% \begin{align*}
%     \DET{\A + \textbf{B}} \geq \DET{\A} + \DET{\textbf{B}}
% \end{align*}
% \end{lemmarep}

\subsection{Privacy Analysis of algorithm \ref{alg:slowlinearbandits}}
% To make the algorithm satisfy zCDP (definition \ref{def:CDP}) we add Gaussian Noise  to each Gram matrix  $\V_t$ to get $\Vtil_t = \V_t + \Z_t$, where $\Z_t$ is the Gaussian Noise Matrix (see definition \ref{def:GNM}). 


We assume that the learner interacts with a single user on each round $t\in[T]$, thus there is a total of $T$ users whose data we want to protect. Each user's data on round $t$  consists of the decision set $\cX_t$ and the reward $y_t$. Therefore we encode a user's $t$ data  with the tuple $u_t = (\cX_t, y_t)$. We say that two user sequences $U=\{u_1, \ldots, u_T\}$, $U'=\{u_1^{'}, \ldots, u_T^{'}\}$ are $t$-neighbors if they are different only in the data of the $t$-th user (i.e., $u_t \neq u_t^{'}$ and  $\forall_{ i\in[T]/\{t\}}  u_i = u_i^{'}$). Our goal is to show that \cref{alg:slowlinearbandits} is jointly-zCDP with respect to neighboring user sequences. 


We follow the billboard lemma as in \cite{hsu2016private}, which says that an algorithm is jointly-zCDP if the output sent to the $i$-th user is a function of the $i$-th user a a signal computed using ZCDP. In algorithm \cref{alg:slowlinearbandits}, the output sent to user $t$ is $\x_t$, which depends only on the private objects $\Vtil_t$ and $\ytil_t$, therefore if can can show that $\Vtil_t$ and $\ytil_t$ satisfy $\rho$-zCDP then we conclude that the algorithm over $T$ rounds satisfies joint $\rho$-zCDP.





\subsection{Regret Analysis}



The regret of linear MAP algorithm is defined as follows

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Def:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{definition} (Pseudo Regret)
Let $\thetabf^*$ be an unknown parameter vector.
Given decision sets, $\cX_1, \ldots, \cX_T$, an agent that chooses actions $\x_t\in\cX_t\subset \mathbb{R}^d$, has pseudo regret 
% of the algorithm can be formally written as:
\begin{equation}
    R(T) = \left( \sum_{t=1}^T \max_{\x\in\cX_t}\vdot{\x, \thetabf^*} \right) - \left( \sum_{t=1}^T \vdot{\x_t, \thetabf^*} \right) = \sum_{t=1}^T \max_{\x\in\cX_t}\vdot{\x- \x_t, \thetabf^*}
\end{equation}
\label{def:pseudo-regret}
\end{definition}


%
%
%%%%%%%%%%%%%%%%%%%%%%%%%
%% Theorem: confidence set 
%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Private Least Squares Confidence Set}
In this section we construct the confidence set of the least squares estimator subject to privacy.
First we give the a bound on the norm on the noise given by the Binary Matrix Mechanism:
\begin{lemmarep}
\label{lem:l2-norm-noise-matrix}
Let $\Z_i \in \mathbb{R}^{d\times d}$ be a random matrix and $\z_i \in \mathbb{R}^d$ a random vector, where each coordinate is sampled i.i.d from the Gaussian distribution with scale $\mathcal{N}\left(0,\frac{L^4}{2\rho}\right)$. Let $\mH_t \in \mathbb{R}^{d\times d}$ be a Binary Gaussian Mechanism matrix, where $\mH_t$ is the sum of at most $\log(T)$ Gaussian noise matrix $\Z_i$. Then, with probability at least $1 - \beta'$ for $\beta' \in (0,1)$, we have: 
\begin{equation}
    \nn{\mH_t}_2 \leq \frac{L^2 \log(T) (4\sqrt{d} + 2\ln(1/\beta'))}{\sqrt{2 \rho}}
\end{equation}

Let $\h_t \in \mathbb{R}^d$ be the sum of at most $\log(T)$ Gaussian noise vector $\z_i$. Then, with probability at least $1 - \beta'$, we have:
\begin{equation}
    \nn{\h_t}_2 \leq \frac{L^2 \sqrt{\log(T)}(\sqrt{d} + \sqrt{2 \ln(1/\beta')})}{\sqrt{2\rho}}
\end{equation}

\end{lemmarep}
\begin{proof}
We begin by sampling a noise matrix $\Z \in \mathbb{R}^{d\times d}$ where each coordinate is drawn i.i.d from $\mathcal{N}\left(0, \frac{L^4}{2\rho}\right)$.


In each round $t$, let the matrix $\mathbf{H}'_t$ be the sum of at most $\log(T)$ Gaussian noise matrices. We want $\mH_t$ to be symmetric, so we let the Binary Gaussian Mechanism matrix $\mH_t = (\mH' + \mH'^\top)/\sqrt{2}$. This transformation preserves the variance of each coordinates in $\mH_t$ to be the same as that of $\mH'_t$. 

Hence, the variance of each coordinate of $\mH_t$ is at most $\frac{L^4 \log(T)}{2\rho}$. 
Then, from \Cref{def:GNM}, with probability at least $1 - \beta'$, the spectral norm of $\mH_t$ is at most:
\begin{align*}
    \nn{\mH_t}_2 \leq\frac{L^2 \log(T) (4\sqrt{d} + 2\ln(1/\beta')) }{\sqrt{2\rho}} 
\end{align*} 

Similarly, $\h_t$ is the sum of at most $\log(T)$ Gaussian random vector $z_i$. Hence, each coordinate of $\h_t$ is a $\chi^2(\log(T))$ random variable. Hence, we can bound the norm of $\h_t$ by:
\begin{align*}
    \nn{\h_t}_2 \leq \frac{L^2}{\sqrt{2\rho}} \sqrt{\log(T)} (\sqrt{d} +  \sqrt{2\ln(1/\beta')}) 
\end{align*}
In the last inequality, we use the following concentration bound on $\chi^2$ random variables: for each coordinate $\h_t^{(i)}$ of vector $\h_t$, with probability $1 - \beta'$, we have 
\begin{align*}
    \h_t^{(i)} \leq \log(T) + 2\sqrt{\log(T) \ln(1/\beta')} + 2\ln(1/\beta')
\end{align*}
\end{proof}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Theorem: confidence
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\privlambda}{\widetilde{\lambda}}
\begin{theoremrep}[Confidence set]
Let $\thetabf^*$ be the vector, such that the rewards are given by
$\y_{1:t} =\pp{  \vdot{\x_1,\thetabf^*} + \eta_1, \ldots, \vdot{\x_t,\thetabf^*} + \eta_t}^\top$ and $\nn{\thetabf^*}_2\leq S$.
%
Let  $\mH_t \in \mathbb{R}^{d\times d}$ be a Binary Gaussian Mechanism matrix and $\h_t\in \mathbb{R}^{d}$ a random vector, where each coordinate is sampled from the Gaussian distribution with scale $\sigma$.
Let $\privlambda\in \mathbb{R}^d$ be such that $\mH_t \prec \privlambda\I$ for all $t\in[T]$, and $\lambda\in \mathbb{R}^d$
%
Let 
\begin{align*}
    \Vtil_t = \X_{1:t}^\top\X_{1:t} + \mH_t +  (\privlambda + \lambda)\I
\end{align*}

%
The private $\ell_2$-regularized least squares estimate of $\thetabf^*$ with parameter $\lambda$, is given by
% Let the center of the confidence set $C_t$ is $\thetahat_t$ and it's defined as
\begin{align*}
    \thetatil_t = \pp{\Vtil_t}^{-1} \pp{\X_{1:t}^\top\y_{1:t} + \h_t}
\end{align*}
For any $\delta>0$,  the  $C_t$ be the confidence set on episode $t$ is given by

\begin{align*}
    C_t=
    \left\{
    \thetabf \in \bbR^d
    : \nn{\thetatil_t - \thetabf}_{\Vtil_t} \leq 
    \beta_{t}(\delta) 
    := R\sqrt{2\log\pp{\frac{\DET{\Vtil_t}^{1/2}\DET{(\privlambda + \lambda)\I}^{-1/2}}{\delta}}} + (\privlambda + \lambda)^{1/2}S
    \right\}
\end{align*}
%
Then with probability at least $1-\delta$,  the vector $\thetabf^* \in C_t$ on all episodes $t\leq T$.
% 
% where $\beta_{t }(\delta) :=  $
\end{theoremrep}
\begin{proof}
Fix round $t\in[T]$.
Let $\X = \X_{1:t}$, $\y = \y_{1:t}$, and $\etabf = (\eta_1,\ldots, \eta_t)^\top$. 
%
By definition, the privatized co-variance matrix is 
$$ \Vtil =  \X^\top\X+\mH_t +  (\privlambda + \lambda)\I$$
and the non-private co-variance matrix is given by $ \V =  \X^\top\X + \lambda\I$. Note that we can choose $\privlambda$ such that $\Vtil \succ \V$. Then, we can expand the least square equation as

\begin{align}
\notag
    \thetatil_t &= \pp{\X^\top\X+\mH_t +  (\privlambda + \lambda)\I}^{-1}
    \pp{
    \X^\top\pp{{\X\thetabf^*}  + \etabf}
    + \h_t
    } \\ 
\notag
    &= {\Vtil}^{-1}
    \pp{\X^\top\etabf + \h_t}
    + {\Vtil}^{-1}\pp{\X^\top \X\thetabf^*} && \text{where } \Vtil =  \X^\top\X+\mH_t +  (\privlambda+\lambda)\I \\ 
    %
\notag
    &= {\Vtil}^{-1}
    \pp{\X^\top\etabf + \h_t}
    + {\Vtil}^{-1}{\Vtil}\thetabf^*
    - {\Vtil}^{-1}\pp{\mH_t +  (\privlambda+\lambda)\I}\thetabf^* \\
     %
     \label{eq:confI}
    &= {\Vtil}^{-1}
    \pp{\X^\top\etabf + \h_t}
    + \thetabf^*
    - {\Vtil}^{-1}\pp{\mH_t +  (\privlambda+\lambda)\I}\thetabf^*
\end{align}


For any $\x \in \bbR^d$, we can multiply both sides of \cref{eq:confI} by $\x^\top$ and we get
\begin{align}
\notag
    &\x^\top \thetatil_t - \x^\top  \thetabf^* \\ 
\notag
    &= \x^\top\Vtil^{-1}\pp{\X^\top\etabf + \h_t}
    -\x^\top\Vtil^{-1}\pp{\mH_t + (\privlambda+\lambda) \I}\thetabf^*\\ 
% \label{eq:confI}
    &= 
    % \x_t^\top\pp{\Vtil_t}^{-1}\pp{\X\eta_t + \h_t}
    \vdot{\x, \X^\top\etabf + \h_t}_{\Vtil^{-1}} 
    - \vdot{\x, \pp{\mH_t + (\privlambda+\lambda) \I}\thetabf^*}_{\Vtil^{-1}} \\
    &= 
    % \x_t^\top\pp{\Vtil_t}^{-1}\pp{\X\eta_t + \h_t}
    \vdot{\x, \X^\top\etabf }_{\Vtil^{-1}} 
    + \vdot{\x,  \h_t}_{\Vtil^{-1}} 
    - \vdot{\x, \mH_t\thetabf^*}_{\Vtil^{-1}} 
    -  (\privlambda + \lambda)\vdot{\x, \thetabf^*}_{\Vtil^{-1}}  
\end{align}

By applying Cauchy-Schwartz inequality we get 
\begin{align}
    % \abs{\vdot{\x, \cX^\top\etabf + \h_t}_{\Vtil^{-1}} }
    \abs{\x^\top \thetatil_t - \x^\top  \thetabf^*}
    &\leq \nn{\x}_{\Vtil^{-1}}
    \pp{
    \nn{ \X^\top\etabf}_{\Vtil^{-1}}
    +
    \nn{\h_t}_{\Vtil^{-1}}
    +
    \nn{\mH_t \thetabf^*}_{\Vtil^{-1}}
    +
   (\privlambda+\lambda) \nn{\thetabf^*}_{\Vtil^{-1}}
    }
\end{align}

For the next step we use
$\privlambda\I + \mH_t \succ 0$, it follows that  
$\X^\top\X+\mH_t +  (2\privlambda+\lambda)\I \succ  \X^\top\X+ (\privlambda + \lambda)\I $. Hence, we have $\lambda_{\min}(\Vtil) = \privlambda + \lambda$.

Now we focus on bounding the term $(\privlambda+\lambda) \nn{\thetabf^*}_{\Vtil^{-1}}$. We use $\nn{\thetabf^*}^2_{\Vtil^{-1}} \leq \tfrac{1}{\lambda_{\text{min}}(\Vtil) } \nn{\thetabf^*}_2^2$.

\begin{align}
   (2\rhomax+\lambda) \nn{\thetabf^*}_{\Vtil^{-1}}\leq 
   (\rhomax+\lambda)^{1/2} S
\end{align}

Next we bound $\nn{\h_t}$ and $ \nn{\mH_t \thetabf^*}$. \gv{TODO: Bound these two terms. See \cite{shariff2018differentially}. The upper bound should be in the order of $\nn{\mH_t \thetabf^*}\leq O(\sqrt{d}\rhomax)$  and $\nn{\h_t}\leq O(d\rhomax)$, where $d$ is the dimension and $\rhomax$ is the scale of the Gaussian noise added to each coordinate. Add as a separate Lemma.}

operator norm: $\|v\|_{op} = \max_{x:\|x\|_2\leq 1 } \langle v, x \rangle $ 

Let $\V = \X^\top \X + \lambda \I$.
Note that $\V \succ \I$, then $\Vtil = \V + \mH + \privlambda \I$

\paragraph{Bound $ \nn{\h_t}_{\Vtil^{-1}}$} 

We know that $ \X \X^\top + \lambda\I\succ 0$ is true.

So If we set $\V = \X \X^\top + 2\lambda\I$. 

Then $\V - \lambda\I \succ 0$.


\begin{align*}
   \nn{\h_t}_{\Vtil^{-1}}
   =\nn{\h_t}_{\pp{\V + \mH_t + \privlambda\I}^{-1}}
   \leq \nn{\h_t \thetabf^*}_{\V^{-1}}
\end{align*}


\paragraph{Bound $\nn{\mH_t \thetabf^*}_{\Vtil^{-1}}$:}
\begin{align*}
    \nn{\mH_t \thetabf^*}_{\Vtil^{-1}}
    &= \nn{\mH_t \thetabf^*}_{\pp{\V + \mH_t + \privlambda\I}^{-1}}
    \leq  \nn{\mH_t \thetabf^*}_{\V ^{-1}}
    \leq  \nn{\mH_t \thetabf^*}_{\pp{\I}^{-1}}
    \leq  S \nn{\mH_t}\\
    &\leq S \frac{L^2 \log(T)(4\sqrt{d} + 2\ln(1/\beta'))}{\sqrt{2\rho}} \tag{by \Cref{lem:l2-norm-noise-matrix}}
\end{align*}





Lastly we bound $\nn{ \X^\top\etabf}_{\Vtil^{-1}}$ using the techniques from \cite{abbasi2011improved}.

% \begin{align}
% \x^\top\left(\Vtil^{-1}\pp{\mH_t + (\rhomax+\lambda) \I}\right)\thetabf^* 
% %
% &\leq (2\rho + \lambda) \x^\top\Vtil^{-1}\thetabf^*  \\ 
% %
% %
% & =  (2\rho + \lambda) \vdot{\x,\thetabf^*}_{ \Vtil^{-1} }  \\ 
% %
% % &= \vdot{\x, \Vtil^{-1} \thetabf^*}_{(2\rhomax+\lambda) \I}  \\ 
% % %
% % &\leq 
% % \abs{ \vdot{\x, \thetabf^*}_{\pp{\A^\top\A+\lambda\I}^{-1}\pp{ (2\rhomax+ \lambda) \I}} } \\ 
% % &= 
% % \abs{(2\rhomax+ \lambda) \vdot{\x, \thetabf^*}_{\pp{\A^\top\A+\lambda\I}^{-1} }}\\
% % &\leq 
% % \sqrt{(2\rhomax+ \lambda)}
% %  \nn{\x}_{\pp{\A^\top\A+\lambda\I}^{-1}}
% % \nn{\thetabf^*}_{\pp{\A^\top\A+\lambda\I}^{-1} }
% \end{align}

\end{proof}





%
%
%
\begin{lemmarep}
Let $\{\x_t\}^{\infty}_{t=1}$ be a sequence in $\mathbb{R}^d$,  define $\Vtil_t = \sum_{i=1}^{t} \x_i \x_i^\top + \mH_t$ and parameter $\lambda$, such that $\mH_t + \lambda\I \succ 0$. Then, we have that:
\gv{Add $\privlambda$}
%
\begin{align*}
    \log\left(\frac{\det(\Vtil_t + \lambda\I)}{\det(\lambda\I)} \right) \leq \sum_{i=1}^t \nn{\x_i}^2_{\Vtil_{i-1}^{-1}}
\end{align*}
Furthermore, if $\nn{\x_t}_2 \leq L$ for all $t$, then
%
\begin{align*}
    \sum_{i=1}^t \min \{1 , \nn{\x_t}^2_{\Vtil_{t-1}^{-1}} \} \leq 2(\log\det(\Vtil_t + \lambda\I) - \log\det(\lambda\I)) \leq 2(d\log((\mathrm{tr(\mH_t + \lambda\I)} + t L^2)/d) - \log\det(\lambda\I)) \\ 
    \leq 2((d\log((2d \lambda) + t L^2)/d) - \log\det(\lambda\I))
\end{align*}
\label{lem:sum-norm-bound}
\end{lemmarep}
\begin{proof}
Using algebra, we have:
\begin{align*}
    \DET{\Vtil_t + \lambda \I} &= \DET{\Vtil_{t-1} + \x_t \x_t^\top}\\
    &= \DET{\Vtil_t} \DET{\I + \Vtil_{t-1}^{-1/2} \x_t (\Vtil_t ^{-1/2}\x_t^\top)}\\
    &= \DET{\Vtil_{t-1}}(1 + \nn{\x_{t-1}}^2_{\Vtil_{t-1}^{-1}})\\
    &= \DET{\lambda \I} \prod_{i=1}^t \left( 1 + \nn{\x_t}^2_{\Vtil_{i-1}^{-1}} \right)
\end{align*}
Taking $\log$ from both sides, we have:
\begin{align*}
    \log\DET{\Vtil_t} &\leq \log\DET{\lambda \I} + \sum_{i=1}^t \log \left( 1 + \nn{\x_t}^2_{\Vtil_{i-1}^{-1}} \right)\\
    &\leq \log\DET{\lambda \I} + \sum_{i=1}^t \nn{\x_t}^2_{\Vtil_{i-1}^{-1}} \tag{since $\log(1 + t) \leq t$}
\end{align*}
Notice that $t \leq 2 \log(1 + t)$ when $x \in [0,1]$. We have:
\begin{align*}
    \sum_{i=1}^t \min \{1, \nn{\x_i}^2_{\Vtil_{i-1}^{-1}} \} &\leq 2 \sum_{i=1}^t \log (1 + \nn{\x_i}^2_{\Vtil_{i-1}^{-1}})\\
    &= 2(\log \DET{\Vtil_t + \lambda \I} - \log \DET{\lambda \I})
\end{align*}
Observe that 
\begin{align*}
    \log \DET{\Vtil_t + \lambda \I} &= \log(\prod_{i=1}^d \lambda_i)\\
    &\leq \log \left( \left( \right)^d \right)\\
    &\leq d \log \left(\frac{\mathrm{tr}(\Vtil_t + \lambda \I)}{d} \right)\\
    &= d \log \left( \frac{\mathrm{tr}(\V_t + \mH_t + \lambda \I)}{d}\right)\\
    &\leq d \log \left( \frac{\mathrm{tr}(\mH_t + \lambda \I)+ tL^2}{d} \right) \tag{since $\mathrm{tr}(\V_t) \leq tL^2$}
\end{align*}
With large enough $\lambda$, we also have $\mathrm{tr}(\mH_t) \leq \mathrm{tr}(\lambda \I) = d \lambda$. Substitute this expression into the inequality above, we have:
\begin{align*}
    \log \DET{\Vtil_t + \lambda \I} \leq d \log \left( \frac{2d \lambda+ tL^2}{d} \right) 
\end{align*}
\end{proof}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Sub-Section: Regret
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Private MAP Regret}

\begin{lemmarep}
\label{lem:sup-det-bound}
Let $\cX, \textbf{B}$ and $\textbf{C}$ be positive semi-definite matrices such that $\cX = \textbf{B} + \textbf{C}$. Then, we have that 
\begin{align*}
    \sup_{\x \neq 0} \frac{\x^\top \cX \x}{\x^\top \textbf{B} \x} \leq \frac{\det(\cX)}{\det(\textbf{B})}
\end{align*}
\end{lemmarep}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% [Generic regret]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theoremrep}[Generic regret]
Assume that:
\begin{itemize}
    \item for all $t$ and all $\x \in \cX_t$, $\vdot{\x, \thetabf^*} \in [-1, 1]$ and $\|\thetabf^\star\|\leq S$.
    \item If for all $t\in[T]$ w.p. at least $1-\delta$,  $\|\thetabf^*-\thetatil_t\|_{\Vtil_t + \lambda \I} \leq \beta_t(\delta)$
    and  $\beta_1\leq \ldots, \leq \beta_T$
    \item If $t$ is the current episode and  $k$  the last update index then $\frac{\DET{\Vtil_t + \lambda\I} }{\DET{\Vtil_k+ \lambda\I} } < C$
\end{itemize}
%
Then, with probability at least $1-\delta$, the regret of \cref{alg:slowlinearbandits} with update rate $C>1$ satisfies
%
\begin{align*}
    R(T) \leq 2\beta_T\sqrt{2C T((d\log((2d \lambda) + t L^2)/d) - \log\det(\lambda\I))}
\end{align*}
\end{theoremrep}
%
\begin{proof}
For a time $t$, let $\tau_t $ be the time of the last trigger event before $t$ or $0$ if $t$ is the first trigger event. Then, we can write the instantaneous regret at round $t$ as: 
\begin{align*}
    r_t &= \vdot{\x^*, \thetabf^*} - \vdot{\x_t, \thetabf^*}\\
    &\leq \vdot{\x_t, \thetatil^{(+)}_{\tau_t}} - \vdot{\x_t, \thetabf^{*}}\\
    &= \vdot{\x_t, \thetatil^{(+)}_{\tau_t} - \thetabf^*}\\
    &= \vdot{\x_t, \thetatil_{\tau_t} - \thetabf^*} + \vdot{\x_t, \thetatil^{(+)}_{\tau_t} - \thetatil_{\tau_t}}
\end{align*}
For all $\thetabf \in C_{\tau_t}$ and any $\x \in \cX_t$, we have:
\begin{align*}
    \abs{\x^\top (\thetabf - \thetatil_{\tau_t})}
    &\leq \nn{(\Vtil + \lambda \I)^{1/2}_t (\thetabf - \thetatil_{\tau_t})} \sqrt{\x^\top (\Vtil_t + \lambda \I)^{-1}  \x} \tag{Cauchy-Schwarz}\\
    &\leq \nn{(\Vtil_{\tau_t} + \lambda \I)^{1/2} (\thetabf - \thetatil_{\tau_t})} 
    \sqrt{\frac{\det(\Vtil_t + \lambda \I)}{\det(\Vtil_{\tau_t} + \lambda \I)}} \sqrt{\x^\top (\Vtil_t + \lambda \I)^{-1}\x} 
    \tag{from Lemma \ref{lem:sup-det-bound}}\\
    &\leq \sqrt{C} \nn{(\Vtil_{\tau_t} + \lambda \I)^{1/2}(\thetabf - \thetatil_{\tau_t})}\sqrt{\x^\top (\Vtil_t + \lambda \I)^{-1}\x} \tag{since $C \geq \frac{\det(\Vtil_t z= \lambda \I)}{\det(\Vtil_{\tau_t + \lambda \I})}$}\\
    %
    &= \sqrt{C} \nn{\thetabf - \thetatil_{\tau_t}}_{\Vtil_{\tau_t} + \lambda \I} \nn{\x}_{(\Vtil_{t} + \lambda \I)^{-1}} \\
    %
    &\leq  \sqrt{C}\beta_{\tau_t}\nn{\x}_{(\Vtil_{t} + \lambda \I)^{-1}}
\end{align*}


Since we also have $r_t \leq 2$, we can write:
\begin{align*}
    r_t &\leq 2 \min( \sqrt{C} \beta_{\tau_t}\nn{\x}{(\Vtil_{t} + \lambda \I)^{-1}} , 1)\\
    &\leq 2\sqrt{C} \beta_{\tau_t}\min(\nn{\x_t}_{(\Vtil_{t} + \lambda \I)^{-1}}, 1)
\end{align*}
Hence, for probability at least $1 - \delta$, for all $T \geq 0$, we have:
\begin{align*}
    R(T) \leq &\sqrt{T \sum_{t=1}^T r_t^2 } \\ 
    \leq& \sqrt{T \sum_{t=1}^T  4 C\beta_{\tau_t}^2\min(\nn{\x_t}_{(\Vtil_{t} + \lambda \I)^{-1}}^2, 1) }\\
    \leq& \sqrt{T \sum_{t=1}^T  4 C\beta_{T}^2\min(\nn{\x_t}_{(\Vtil_{t} + \lambda \I)^{-1}}^2, 1) }\tag{Assumption 2} \\
    \leq& 2\beta_T\sqrt{C T \sum_{t=1}^T \min(\nn{\x_t}_{(\Vtil_{t} + \lambda \I)^{-1}}^2, 1) }\\
    \leq& 2\beta_T\sqrt{C T [\log\det(\Vtil_T + \lambda \I) - \log\det(\lambda \I) ]} \tag{from Lemma \ref{lem:sum-norm-bound}}\\
    \leq& 2\beta_T\sqrt{2C T((d\log((2d \lambda) + t L^2)/d) - \log\det(\lambda\I))}
\end{align*}
\end{proof}


% im moving this section up


==> files/LinearMAB/lazy_mab.tex <==

\section{Slowly Updating Linear Stochastic Bandits }\label{sec:linearbandits}




\newcommand{\epsG}{\epsilon_{\text{G}}}
\newcommand{\epsS}{\epsilon_{\text{S}}}
\begin{algorithm}[H]
\SetAlgoLined
\textbf{Parameters: } Privacy parameter $\rho$, noise scale $\sigma$,  regularization $\lambda$, update rate $c$. \\
%

% $\epsG \leftarrow \text{ Parameter of the Gaussian Mechanism .} $ \\
% $\epsS \leftarrow \text{Parameter of  the Above Threshold Mechanism} $ \\
%
%
% Let $\rhomax \leftarrow  2\frac{\sqrt{d}L}{\sqrt{\rho}}$ \\ 
% $\V_0 \leftarrow (\rhomax + \lambda) I$ and $\y_0 \leftarrow 0_\text{d}$ \\
Let $k\leftarrow 1 $ \tcp*{Last time the policy was updated.}

% Let $\widetilde{c}_\tau = c\DET{\V_0} + \mathrm{Lap}(\frac{2}{\epsS}) $ \\
%
Set $\V_1 \leftarrow 0_{d\times d}$;\\
Set $\y \leftarrow 0_d$;\\
%
\For{$t=1, \dots, T-1$}{
    \label{alg:doubledet}
    
    \If{$\DET{\Vtil_{t} + \lambda\I } \geq  c \DET{\Vtil_{k}+ \lambda\I }$}{
        % Let $\Vtil_{t} \leftarrow \V_{1:k} + \V_{k:t} + \Gau\pp{\sigma}$ 
        % Let $\Vtil_{t} \leftarrow \Vtil_{k:t} + \Vtil_k$  
        % and $\ytil_t \leftarrow \y_t + \Gau\pp{\sigma}$\\
        % 
        Compute least square estimate: $\thetatil_{t} \leftarrow \pp{\Vtil_{t} + \lambda\I}^{-1}  \ytil_{t}$ and $\beta(\cdot)$ \\ 
        % Construct confidence set $C_t = \left\{ \thetabf : \nn{\thetabf - \thetatil_{t}}_{\Vtil_{t}} \leq \sqrt{\beta_t} \right\}$ \\
        %
        % Update $\widetilde{c} =     
        Update index: $k\leftarrow t$ \tcp*{update index}
        % Update threshold for $\AT$:  \\
        % $\mathrm{Thres}_k \leftarrow \DET{\Vtil_k +  \lambda\I} + \text{Lap}\pp{\frac{2}{\sqrt{2\rho}} }$  \\
        % \tcp*{$\Vtil_k $ is private.} 
        % {\color{blue} $\mathrm{Thres}_k \leftarrow \DET{\V_k +  \lambda\I} + \text{Lap}\pp{\frac{2}{\sqrt{2\rho}} }$}
        % $\mathrm{Thres} \leftarrow \DET{\Vtil_k} + \mathrm{Lap}(\frac{2}{\epsS})$
    }
    
    Observe decision set $\cX_t$. \\
    % // Let $\x_t,\thetatil^{(+)}_t \leftarrow  \argmax_{\x\in\cX_t}\argmax_{\theta \in  C_{k}} \vdot{\theta, \x}$\\ 
    $\x_t \leftarrow \argmax_{\x\in \cX_t} \vdot{\thetatil_k, \x} + \beta_k \nn{\x}_{\Vtil_{k}^{-1}}$
    \tcp*{choose best action.}
    Play $\x_t$ and observe reward $r_t$ \\
    %
    Update: $\V_{t+1} \leftarrow \V_{t} + \x_t  \x_t^\top$ \text{ and }
     $\y_{t+1} \leftarrow \y_{t} + \x_t r_t$ \\
    %
    Binary Mechanism: $\Vtil_{t+1} \leftarrow \V_{t+1} + \Z_{t+1}$ and  $\ytil_{t+1} \leftarrow \y_{t} + \z_{t+1}$
}   
\caption{Slowly Updating DP-UCB}\label{alg:slowlinearbandits}
\end{algorithm}

==> files/LinearRL/algorithm.tex <==
\section{JDP RL with Low Switching Cost}

We now introduce our RL algorithm for the linear MDP setting. Before we introduce our private algorithm, we will first revisit the non-private algorithm of Least-Squares Value Iterations (LSVI) and then introduce our techniques to make such an algorithm private with a desirable privacy-accuracy trade-off.

\paragraph{LSVI}

In the linear MDP setting, we leverage the fact that the action value function $Q_h^\star$ is linear in the feature vector (Proposition \ref{prop:linear-func}) and thus they can be estimated using the idea of Least-Squares Value Iterations \citep{bradtke1996linear, osband2016generalization}. In particular, the true action-value function $Q_h^\star$ is parameterized by a vector $\w_h^\star$. If we updated the policy on episode $k$, then \cref{alg:privrl} recursively estimates  $\w_h^\star$ for all $h$ using a LSVI. Let $Q_h^k$ and  $\w_h^k$ denote the running estimates of the action-value functions and their corresponding parameters over episodes.
In each episode $k$, the algorithm computes the following sufficient statistics relevant to the estimation of $\w_h^\star$: starting with $h = H$ down to $h=1$, compute
a least-squares estimate $\w_h^k$ via
\begin{align}
\label{eq:lambdadef}
\LambdaMAT_h^k &= {\sum_{i=1}^{k-1} \phib{x_h^i,a_h^i}\phib{x_h^i,a_h^i}^\top
    } \\
\label{eq:ydef}
    \y_h^k &= {\sum_{i=1}^{k-1} \phib{x_h^i,a_h^i} \pp{r_h^i + V_{h+1}^{k}(x_{h+1}^i)}}\\
    \w_h^k &= \left(\LambdaMAT_h^k\right)^{-1}  \y_h^k,
\end{align}
which subsequently define the corresponding optimistic estimates for action-value and state-value functions:
\begin{align}
Q_h^k(x, a) &= \langle \phi(x, a), \w_h^k\rangle +  \beta\|\phib{\cdot, \cdot}\|_{\pp{\LambdaMAT_h^k}^{-1}}\\
V_h^k(x) &= \max_a Q_h^k(x, a)
\end{align}
% Given the estimate $\w_h^k$, the algorithm computes the optimistic action-value function $Q_h^k(\cdot, \cdot) = \vdot{\phib{\cdot, \cdot}, \w_h^k} $, where $\beta$ is a bonus term that ensures optimism. The non-private algorithm follows a greedy policy with respect to the estimates of action-value functions. 
Given these optimistic estimate, the non-private algorithm follows a greedy policy with respect to the estimates of action-value functions. 

%
% That is,  starting with $h=H$ down to $h=1$, let $\w_h^{k}$ be the privacy-preserving approximation of $\w_h^\star$, given by $\w_h^{k} = \pp{\Lambtil_h^{k}}^{-1}\ytil_h^{k}$.

% Given the parameter $\w_h^k$, the algorithm computes the optimistic action-value function $Q_h^k(\cdot, \cdot) = \vdot{\phib{\cdot, \cdot}, \w_h^k} + \beta\|\phib{\cdot, \cdot}\|_{\pp{\Lambtil_h^k}^{-1}}$, where $\beta$ is a bonus term that ensures optimism. Then the algorithm recursively computes $\w_{h-1}^k$, with $V_h^k(x) = \max_a Q_h^k(x, a)$.









\paragraph{Private LSVI-UCB} 
In order to provide a JDP variant of the LSVI algorithm, our strategy is to identify a collection of statistics that are compatible with differentially private releases and sufficient for constructing estimates for the action value functions. In this case,  it is sufficient to release of the set of sufficient statistics $\{\LambdaMAT_h^k, \y_h^k\}_{k,h \in [K] \times [H]}$ subject to DP. 


% that are used to maintain and update a running optimistic estimate of the action-value function, denoted by $Q_h^k$, which in turn gives the corresponding estimates for value functions $V_h^k$. For each time step $h\in [H]$,
% the Gram matrix $\LambdaMAT_h^k$ and the vector $\y_h^k$ are defined as:
% the variable $\LambdaMAT_h^k$ is the Gram matrix given by the relevant observed feature vectors $\phi(x_h^i, a_h^i)$ so far, and $\y_h^k$ is the target vector in the relevant least-squares regression problem, defined below:


 In order to preserve privacy, \cref{alg:privrl} adds noise to the sufficient statistics, which we denote by $\{\Lambtil_h^k, \ytil_h^k\}_{k,h \in [K] \times [H]}$, where 
\begin{align}
\label{eq:lambdatildef}
    \Lambtil_h^{k} &= {\LambdaMAT_h^k} + 2\binmechboundvar\I + \M_h^k \\
\label{eq:ytildef}
    \ytil_h^k &= {\y_h^k} + \etabf_h^k
\end{align}
and  $\{\M_h^k, \y_h^k\}_{k,h\in[K]\times [H]}$ are noise injected to privatize the statistics. 
To guarantee that the noise matrix $\M_h^t$
in \cref{eq:lambdatildef} is positive definite, we shift it by $2\binmechboundvar\I$. Now we show how to release these two types of statistics ${\LambdaMAT_h^k}$ and $\y_h^k$ at a low privacy cost.

\input{../files/LinearRL/pseudocode}
% \input{../files/LinearRL/pseudocode_icml}

\paragraph{Binary Mechanism} We first introduce the mechanism to privatize the sequence of Gram matrices $\LambdaMAT_h^k$. First, notice that the Gram matrix statistic is in form of a sum. This allows us to use a variation of the binary  mechanism due to \cite{shariff2018differentially}, which is a tree-based aggregation mechanism that sequentially releases sums of matrices privately. We initialize $H$ private counters $\cC_h$, for $h\in[H]$. Each counter $\cC_h$ maintains a binary tree in which each internal node represents a partial sum denoted by $\Sigma[i,j] = \sum_{k=i}^j \phib{x_h^k, a_h^k}\phib{x_h^k, a_h^k}^\top$, and each leaf node represents a sum with a single episode. To compute $\LambdaMAT_h^k$, the counter $\cC_h$ sums up the noisy partial-sums that cover the range $[1, k-1]$. Any single data point appears in at most $\log(K)$ nodes of $\cC_h$, hence if each partial sum satisfies $\pp{\rho/ \log(K)}$-zCDP, then by composition the entire algorithm satisfies $\rho$-zCDP.
%

%
% Introduce the adaptive policy updates idea and why we need it.
\paragraph{Gaussian mechanism with low switching cost}
Our second set of statistics  $\y_h^k$ do not take the form of summation, as it contains the value function estimate $V_{h+1}^k$, which is defined as a maximization over  estimates $Q_{h+1}^k(\cdot, a)$. As a result, we cannot apply binary mechanism. Therefore, on each update episode, we use the Gaussian mechanism to privatize $\ytil_h^k$. However, adding Gaussian noise to every episode would lead to too much noise. For this reason, we minimize the number of episodes we update the policy. 

In \cref{alg:privrl}, an update episode occurs every time the determinant of the noisy gram matrix $\Lambtil_h^k$ doubles for any $h \in [H]$. Since \cref{alg:privrl} does not update the action-value function every round, we use $\tilde{k}$ to denote the last episode the policy $\pi_h^k$ was updated. 
% Therefore, the action-value function on episode $k$ and time $h$ is given by $Q_h^k(\cdot, \cdot) = \vdot{\phi(\cdot, \cdot), \w_h^{\tilde{k}_h}} $. 

As shown in \cite{wang2021provably}, this adaptive update schedule allows us to bound the number of policy updates by $O(dH\log(K))$ while increasing the regret only by a factor of $2$. Therefore, instead of applying composition over $K$ Gaussian mechanisms, we only have $O(dH^2\log(K))$. Having $O(\log(K))$ updates is critical for obtaining our improved regret rate. The algorithm from \cite{luyo2021differentially} uses a non-adaptive batching technique that leads to a number of updates polynomial in $K$. In the next section, we show how to analyze the privacy guarantee of this adaptive update algorithm. 
%
% For any episode $k\in[K]$, 



\input{files/LinearRL/switching_cost}




% We ran into a block trying to bound the sensitivity of the sufficient statistics for the MDP. 

% The problem is that the data of each user depends on the policy. So if we change the data of user $t$, then the policy of future episodes will generate different data. 

% For example, let's say that we have two $t$-neighboring user sequences $U, U'$ and  we want to estimate the average reward up to episode $T$. Then the sequence of rewards is going to be different under $U$ and $U'$ after episode $t$, because the agent is following a different policy after episode $t$.

% I think we saw this in the first RL paper but I don't remember how we resolved this. 


==> files/LinearRL/conclusion.tex <==
\section{Conclusion and Future Works}
In this paper, we present a differentially private algorithm in the linear MDP setting with improved regret guarantee. The key component of our analysis is an adaptive update schedule, that only updates a policy when sufficient changes have been observed in the data. Hence, we can leverage this low switching cost paradigm and only perform $O(dH \log(K))$ policy updates, leading to $\widetilde{O} (\sqrt{d^3 H^4 K} + \frac{H^2 d^{5/4} K^{1/2}}{\epsilon^{1/2}})$ regret. Our private regret does not dominate the non-private regret, and improves upon prior works guarantee in all relevant parameters. 

We also provide some future directions: 
\begin{itemize}
    \item 
\end{itemize}

==> files/LinearRL/lemmas/B4_v2.tex <==
\begin{lemma}[(B4 version 2)Similar to Lemma B.4 in \cite{jin2020provably}] 
\label{lem:B4}
Under event $\mathcal{E}$, 
% There exists a constant $c_\beta$ such that $\beta = c_\beta dH\sqrt{\iota}$ where $\iota = log(dT/p)$, and 
for any fixed policy $\pi$, on the event $\mathfrak{E}$ defined in \cref{lem:B3}, we have for all $(x,a,h,k)$ that:
%
\begin{align*}
    \vdot{\phi(x,a), \w_h^{\tilde{k}}} - Q_h^\pi 
    % Q_h^t(x,a) - Q_h^\pi (x,a)
    =\bbP_h\pp{\V_{h+1}^k - \V_{h+1}^\pi}(x,a) + \Delta_h^k(x,a)
\end{align*}
for some $\Delta_h^k(x,a)$ that satisfies $|\Delta_h^k(x,a)| \leq \beta \sqrt{\phi(x,a) (\Lambtil_h^{\tilde{k}})^{-1}\phi(x,a)^\top}$.
\end{lemma}

==> files/LinearRL/lemmas/B4_v2_proof.tex <==
\begin{proof}

By \Cref{prop:linear-func} and the Bellman equation, we have that for any tuple $(x,a,h) \in \mathcal{S} \times \mathcal{A} \times [H]$:
\begin{equation*}
    Q^{\pi}_h (x,a) := \langle \phi(x,a), \w_h^{\pi} \rangle = (r_h + \bbP_h V^{\pi}_{h+1})(x,a)
\end{equation*}

For any $k\in[K]$, the value function is \cref{alg:privrl} is defined as
\begin{align*}
    Q_h^k(x,a) = \vdot{\phi(x,a), \w_h^{\tilde{k}}}, \text{ where } 
    \w_h^{\tilde{k}} = \pp{\Lambtil\ii{\tilde{k}}{h}}^{-1}\widetilde{\y}_h^{\tilde{k}} 
\end{align*}
Note that $\tilde{k} \leq k$ is the last update episode for any $h\in[H]$ before episode $k$.

%%%%% %%%%% %%%%% 
%% Definitions:
%%%%% %%%%% %%%%% 

\begin{align*}
    \Lambtil\ii{k}{h} =
    (\lambda+\lambtil)\I + 
    \sum_{i=1}^{\tilde{k}-1} \phi\pp{x\ii{i}{h}, a\ii{i}{h}}\phi\pp{x\ii{i}{h}, a\ii{i}{h}}^\top 
    +\M\ii{i}{h}, \text{ and } \\
    %
    \ytil_h^k = \sum_{i=1}^{\tilde{k}-1}\phib{x\ii{i }{h}, a\ii{i}{h}} 
    \left( 
    r_h(x\ii{i }{h}, a\ii{i}{h}) + 
    V_{h+1}^{\tilde{k}}(x_{h+1}^i)
                \right) + \eta_h^{\tilde{k}}
\end{align*}

Hence, we have
\begin{align*}
    &\quad \w^{\tilde{k}}_h - \w^{\pi}_h\\
    &= (\Lambtil^{\tilde{k}}_h)^{-1} \pp{\sum_{i=1}^{{\tilde{k}}-1} \phi^i_h [r^i_h + V^{\tilde{k}}_{h+1}(x^i_{h+1})] + \eta_h^{\tilde{k}}} - \w^{\pi}_h\\
    %
     &= (\Lambtil^{\tilde{k}}_h)^{-1} \pp{\sum_{i=1}^{{\tilde{k}}-1} \phi^i_h [r^i_h + V^{\tilde{k}}_{h+1}(x^i_{h+1})] } - \w^{\pi}_h + \pp{\Lambtil_h^{\tilde{k}}}^{-1} \eta_h^{\tilde{k}} \\
    %
    &= (\Lambtil^{\tilde{k}}_h)^{-1} \left( \sum_{i=1}^{\tilde{k} - 1} \phi_h^i r_h^i + \sum_{i=1}^{\tilde{k} - 1} \phi_h^i V_{h+1}^{\tilde{k}}(x_{h+1}^i) + \phi_h^i \bbP_h V_{h+1}^{\pi} (x_h^i, a_h^i) - \phi_h^i \bbP_h V_{h+1}^{\pi}(x_h^i, a_h^i) \right) - \w^{\pi}_h + \pp{\Lambtil_h^{\tilde{k}}}^{-1} \eta_h^{\tilde{k}}\\
    &= (\Lambtil^{\tilde{k}}_h)^{-1} \left(\sum_{i=1}^{\tilde{k} - 1} \phi_h^i \left(r_h^i + \bbP_h V_{h+1}^{\pi}(x_h^i, a_h^i) \right) + \sum_{i=1}^{\tilde{k} - 1} \phi_h^i \left( V_{h+1}^{\tilde{k}}(x_{h+1}^i) - \bbP_h V_{h+1}^{\pi}(x_h^i, a_h^i) \right) \right) - \w_h^{\pi} + \pp{\Lambtil_h^{\tilde{k}}}^{-1} \eta_h^{\tilde{k}}\\
    &= (\Lambtil^{\tilde{k}}_h)^{-1} \left(\sum_{i=1}^{\tilde{k}-1} \phi_h^i \langle \phi_h^i, \w_h^{\pi} \rangle + \sum_{i=1}^{\tilde{k} - 1} \phi_h^i \left( V_{h+1}^{\tilde{k}}(x_{h+1}^i) - \bbP_h V_{h+1}^{\pi}(x_h^i, a_h^i) \right)  \right) - \w_h^{\pi} + \pp{\Lambtil_h^{\tilde{k}}}^{-1} \eta_h^{\tilde{k}}\\
    &= (\Lambtil^{\tilde{k}}_h)^{-1} \left(\sum_{i=1}^{\tilde{k}-1} \phi_h^i \langle \phi_h^i, \w_h^{\pi} \rangle - \Lambtil_h^{\tilde{k}} \w_h^{\pi} + \sum_{i=1}^{\tilde{k} - 1} \phi_h^i \left( V_{h+1}^{\tilde{k}}(x_{h+1}^i) - \bbP_h V_{h+1}^{\pi}(x_h^i, a_h^i) \right)  \right) + \pp{\Lambtil_h^{\tilde{k}}}^{-1} \eta_h^{\tilde{k}}\\
    % (7)
    &= (\Lambtil^{\tilde{k}}_h)^{-1} \left(\sum_{i=1}^{\tilde{k}-1} \phi_h^i \langle \phi_h^i, \w_h^{\pi} \rangle - \left(
    (\lambda+\lambtil) \I + \sum_{i=1}^{\tilde{k}-1} \phi_h^i {\phi_h^i}^\top +  \M_h^i \right) \w_h^{\pi} + \sum_{i=1}^{\tilde{k} - 1} \phi_h^i \left( V_{h+1}^{\tilde{k}}(x_{h+1}^i) - \bbP_h V_{h+1}^{\pi}(x_h^i, a_h^i) \right)  \right) + \pp{\Lambtil_h^{\tilde{k}}}^{-1} \eta_h^{\tilde{k}}\\
    % (8)
    &= (\Lambtil^{\tilde{k}}_h)^{-1} \left\{ \left(-(\lambda+\lambtil) \I - \sum_{i=1}^{\tilde{k}-1} \M_h^i \right) \w_h^{\pi}  + \sum_{i=1}^{{\tilde{k}}-1} \phi^i_h [V^{\tilde{k}}_{h+1}(x^i_{h+1}) - \bbP_h V^{\pi}_{h+1}(x^i_h, a^i_h)] \right\} + \pp{\Lambtil_h^{\tilde{k}}}^{-1} \eta_h^{\tilde{k}} \\
    %
    %
    &= \underbrace{-(\Lambtil_{h}^{\tilde{k}})^{-1} \left( (\lambda + \lambtil)\I + \sum_{i=1}^{\tilde{k}} M_h^i \right)\w_h^{\pi}}_{\textbf{q}_1} + \underbrace{(\Lambtil^{\tilde{k}}_h)^{-1} \sum_{i=1}^{{\tilde{k}}-1} \phi^i_h [V^{\tilde{k}}_{h+1} (x^i_{h+1}) - \bbP_h V^{\tilde{k}}_{h+1}(x^i_h, a^i_h)]}_{\textbf{q}_2} + \\
    %
    %
    &\quad + \underbrace{(\Lambtil_h^{\tilde{k}})^{-1} \sum_{i=1}^{{\tilde{k}}-1} \phi^i_h \bbP_h (V^{\tilde{k}}_{h+1} - V^{\pi}_{h+1}) (x^i_h, a^i_h)}_{\textbf{q}_3}  + \underbrace{\pp{\Lambtil_h^{\tilde{k}}}^{-1} \eta_h^{\tilde{k}}}_{\textbf{q}_4}
\end{align*}

We bound each term individually. First consider the case when $\lambtil \I  \succ \LambdaMAT_k^h$.
 



\end{proof}

==> files/LinearRL/main.tex <==



%%%% Conclusion TDB %%%%
% \input{files/LinearRL/conclusion}

==> files/LinearRL/privacy.tex <==

\subsection{Privacy Analysis}\label{sec:privacy}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Theorem
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \dncomment{translate to $\rho$-zCDP}
% \begin{lemma}[Privacy counter \cite{shariff2018differentially, luyo2021differentially}] 
% Let $T$ be a complete binary tree with its leaf nodes being $l_1, l_2, \cdots, l_n$. Each internal node $x \in T$ stores the sum of all the leaf nodes in the subtree rooted at $x$. Each partial sum $\sum_{j=1}^i l_j$ uses at most $m = \ceil{\log_2(n) + 1}$ nodes of $T$ to its computation. Hence, if each node preserves $(\epsilon_0, \delta_0)$-DP, by advanced composition, the entire algorithm is $(m\epsilon_0^2 + \epsilon_0 \sqrt{2m \log(1/\delta')}, m\delta_0 + \delta')$-DP. Alternatively, to ensure that the tree is $(\epsilon, \delta)$-DP, it suffices to set $\epsilon_0 = \frac{\epsilon}{\sqrt{8m \log(2/\delta)}}$, $\delta_0 = \delta/2m$ (with $\delta' = \delta/2$).
% \end{lemma}


In this section, we provide the privacy analysis of \cref{alg:privrl}. Our main theorem is
\input{files/theorems/jdp/theorem}
% \input{files/theorems/jdp/proof}


For the privacy analysis of \cref{alg:privrl}, we use  zCDP \citep{bun2016concentrated} because it simplifies the composition of Gaussian mechanisms. At the end, we translate our results in terms of DP. In this section, we show that releasing statistics  $\{\Lambtil_h^k\}_{k,h\in[K]\times[H]}$  satisfies $(\rho/2)$-zCDP and then show that releasing $\{\ytil_h^{\tilde{k}}\}_{k,h\in[K]\times[H]}$ also satisfies $(\rho/2)$-zCDP.
%
Thus, by composition of zCDP mechanisms (\cref{lem:zcdpcomposition}), we have that releasing the sufficient statistics satisfies $\rho$-zCDP and, by \cref{lem:cdptodp},  also satisfies $(\epsilon, \delta)$-DP  for $\epsilon = \rho + \sqrt{\rho\log(1/\delta)}$. 

It follows that \cref{alg:privrl} is $\pp{\epsilon, \delta}$-JDP by the Billboard lemma due to \citet{hsu2016private}, since the actions sent to each user depends on a function constructed with DP and their private data only. We state the billboard lemma here:

\input{files/lemmas/billboard/lemma}



% \paragraph{Binary mechanism:} 
% % \gvcomment{gv: Still working on this. Having a hard time with the structure.}
% We now show that releasing the sequence $\{\Lambtil_h^k\}_{k,h}$ satisfies $\rho/2$-zCDP. As in prior work \cite{shariff2018differentially}, we use the Gaussian Binary Matrix Mechanism adapted from \cite{chan2011private}. 
% Each node in the tree represents a partial sum of the form $\sigma[i,j] = \sum_{k=i}^j \phi(x_h^k,a_h^k)$ containing features from episodes $i$ to $j$. 
% Since the noisy partial sums are obtained via Gaussian noise, we have each $\sigma[i,j]$ is $(\Delta^2/2\sigma^2)$-zCDP. Observe that each episode appears in at most $\log(K)$ nodes of the counter $\cC_h$. Hence, by composition, the whole counter $\cC_h$ is $( \log(K)\Delta^2/2 \sigma^2)$-zCDP. 

% % Cut the other two refs from above, since they also cited shariff 

% % \input{files/lemmas/gbmm/lemma}

% % The final privacy guarantee follows from plugging in the  $\ell_2$-sensitivity of $\Lambda_h^k$ for $L$ \swcomment{"final results"?}

% Hence, the counter $\cC_h$ is $(\log(K)/\sigma^2)$-zCDP. Now, we can set $\sigma^2 = \rho/2\log(K)$ to ensure that releasing sequence $\{\Lambtil_h^k \}$ satisfies $\rho/2$-zCDP.

{We start with bounding the sensitivity of the two types of sufficient statistics.}

\input{files/lemmas/sensitivity/lemma}
% \input{files/lemmas/sensitivity/proof}
%

We release these two types of statistics with two mechanisms. First, we use the Gaussian binary mechanism \citep{shariff2018differentially} (a variant of the binary mechanism due to \cite{chan2011private, panprivacy} that preserves positive semi-definiteness in matrices) to privatize the statistics $\{\LambdaMAT_h^k\}_{k,h\in[K]\times[H]}$. For the privacy guarantees, releasing the sequence noisy statistics  $\{\Lambtil_h^k\}_{k,h\in[K]\times[H]}$ using the Gaussian binary matrix mechanism satisfies $(\rho/2)$-zCDP if each partial sum satisfies $(\rho/(2\log(K)))$-zCDP. Since the sensitivity of the Gram matrix is $2$, it suffices to add Gaussian noise to each partial sum with scale $\sigma^2= \frac{4\log(K)}{\rho}$. 


For the remaining of this section, the focus is to show that releasing the statistics $\{\ytil_h^{\tilde{k}}\}_{k,h\in[K]\times[H]}$
also satisfies $(\rho/2)$-zCDP. Recall that, if $\tau$ is an update episode then \cref{alg:privrl} adds Gaussian noise to the statistics $\y_h^\tau$. 
%
Naively, we could update \dndelete{the episode every round}\dnedit{this statistics every episode}, but the noise added would scale with $O(\rho / K)$, giving an error in the order of $O(\sqrt{1/(\rho K)})$, which leads to sub-optimal regret on the variable $K$. Therefore, one would want to update the policy at most $O(dH\log(K))$ times because it allows us to scale the noise with $\rho/\log(K)$, which gives logarithmic error on the parameter $K$. 

The main challenge is that the update episode $\tau$ is a random variable dependent on the user sequence. Thus, any single user in the sequence affects the future update episodes. Therefore, to simplify the analysis, we pretend to run a hypothetical Gaussian mechanism to release a constant function even during rounds in which an update is not triggered.  More formally, for any $h\in[H]$, we construct an adversary that selects an adaptive sequence of functions $f_h^1,\ldots, f_h^K$ as follows: On episode $k$, if $k$ is an update episode then the adversary sets $f_h^k(U_k) = \sum_{i=1}^{k-1} \phib{x_h^i,a_h^i} r_h^i\defeq \y_h^k$ for all $h\in[H]$. Otherwise, the adversary sets $f_h^k(U_k)=0$ for all $h\in[H]$. Note that on non-update episodes, $f_h^k$ is a constant function independent of the data. Also,  \cref{alg:privrl} uses $f_h^k$ only on update episodes to modify the policy and ignores it otherwise. 

The following lemma gives a tool to analyze the protocol under zCDP as long as the joint sensitivity of the sequences $\{f_h^1,\ldots, f_h^K\}_{h\in[K]}$ is bounded. 



\input{files/lemmas/gaussian_adaptive/lemma}
% \input{files/lemmas/gaussian_adaptive/proof}


% Thus, \cref{lem:gaussianadaptivecomp} says that we can release the answers to $f_1,\ldots, f_K$ under zCDP using the Gaussian mechanism with scale equal to the joint sensitivity of $f_1,\ldots, f_K$. 

It only remains to show that the joint sensitivity of the adaptive sequences is bounded. 
First, we show that each $f_h^k$ has bounded sensitivity. By definition of $f_h^k$ and \cref{lem:sensitivity}, we have on any update episode its sensitivity is given by $\Delta(f_h^k) = \Delta(\y_h^k) \leq 3H$  , and on non-update episodes we have that the sensitivity is $\Delta(f_h^k)=0$ for any $h\in [H]$.

Next, we use the fact that number of update episodes in \cref{alg:privrl} is bounded by $\switchcostvar \defeq \switchingcost$ 
% and the sensitivity of $f_h^k$ is bounded by $3H$ (\cref{lem:sensitivity}) for all $k,h\in[K]\times[H]$.
Then the joint sensitivity of the adaptive sequences is given by
\begin{align*}
   \sum_{h = 1}^H \sum_{k=1}^K \Delta(f_h^k) 
   = \sum_{h = 1}^H \sum_{k=1}^K \Delta(\y_h^k) 
   \leq  \sum_{h = 1}^H\Delta(\y_h^k)\switchcostvar \leq 3H^2\switchcostvar
\end{align*}

% if $\Lambtil_h^k \geq C \Lambtil_{\tilde{k}}$ then $k$ is an update episode


Therefore releasing $f_h^k$ with a $\pp{(1/2)\rho / \pp{3H^2\switchcostvar}}$-zCDP Gaussian mechanism on every episode $k\in[K]$ satisfies $\rho/2$-zCDP. This concludes the proof.




==> files/LinearRL/pseudocode.tex <==

\newcommand{\upt}{\textrm{UPDATE}}

% \begin{algorithm}[H]
% \begin{algorithmic}
% % \SetAlgoLined
% % \textbf{Input:} \\
% % \STATE \textbf{Parameters: } 
% \INPUT Privacy parameter $\rho$, policy update rate $C$, fail probability $p$, confidence width $\beta$.
% % Let $M\ii{t}{h} \in \mathbb{R}^{d\times d}$ be the noise from the $\BM$ at episode $t$ for Gram matrix $\Lambda\ii{t}{h}$. \\

% \STATE  $\binmechboundvar \defeq \binmechbound$

% \STATE $\switchcostvar \defeq \switchingcost$ 
% % \COMMENT{Max number of policy updates.}

% \STATE  $\switchcountvar \leftarrow 1$\;

% \STATE  $\rho_0 \leftarrow \rho / (2 \switchcostvar)$
% % \COMMENT{Gaussian mechanism privacy budget.}




% \STATE For all $h\in[H]$,  let $\cC_h{\pp{\frac{\rho}{2H}}}$ be a private counter satisfying $\pp{\frac{\rho}{2H}}$-zCDP.  


% \STATE  $\LambdaMAT\ii{1}{h} \leftarrow  2\binmechboundvar\I,\quad 
% \Lambtil_h^1 \leftarrow \LambdaMAT\ii{1}{h} + \M_h^1$  for all $h\in[H]$\; 

% \STATE  $\tilde{k}_h \leftarrow 1 $  for all $h\in[H]$
% % \COMMENT{Last time the policy was updated.}

% \FOR{$k=1, \dots, K$}
% % {
%     % % \dnedit{
%     % \IF{ $\det\left(\Lambtil\ii{k}{h}\right) \geq C \det\left(\Lambtil\ii{\tilde{k}_h}{h}\right)$}
%     % \STATE add here
%     % \ENDIF
%     % % }

%         \FOR{$h=H\ldots, 1$}
%         % {
        
%             \IF{ $\det\left(\Lambtil\ii{k}{h}\right) \geq C \det\left(\Lambtil\ii{\tilde{k}_h}{h}\right)$
%             \algorithmicand
%             $\switchcountvar < \switchcostvar$
%             } \label{lin:update}
%             % {
%                 % \STATE V_h^{\tilde{k}_h} \leftarrow             
%                 % \STATE $\y_h^k \leftarrow \sum_{i=1}^{k-1}\phib{x\ii{i }{h}, a\ii{i}{h}} 
%                 % ( 
%                 % r_h(x\ii{i }{h}, a\ii{i}{h}) + 
%                 % \max_{a\in\cA}Q_{h+1}^{\tilde{k}_h}(x_{h+1}^i, a)
%                 % )$ 
%                 \STATE $\y_h^k \leftarrow \sum_{i=1}^{k-1}\phib{x\ii{i }{h}, a\ii{i}{h}} 
%                 ( 
%                 r_h^i + 
%                 % \max_{a} Q_{h+1}^{\tilde{k}_h}(x_{h+1}^i, a)
%                 V_{h+1}^{\tilde{k}_h}(x_{h+1}^i)
%                 )$ 
                
%                 \STATE $\widetilde{\y}_h^k \leftarrow \y_h^k + \etabf_h^k $, where $\etabf_h^k \sim \mathcal{N}(0, \frac{2H + 2}{\rho_0})$
                
%                 \label{lin:gaussianmech}
%                 % update w_h
%                 \STATE $\w\ii{k}{h} \leftarrow \pp{\Lambtil\ii{k}{h}}^{-1}\widetilde{\y}_h^k $\;
%                 % Define Q
                
                
%                 % \STATE $Q\ii{k}{h}(\cdot,\cdot) \leftarrow \min\left\{ \vdot{\w\ii{k}{h}, \phib{\cdot, \cdot}} + \beta\left[ \phib{\cdot, \cdot}^\top \left(\Lambtil\ii{k}{h}\right)^{-1}\phib{\cdot, \cdot}   \right]^{1/2}, H\right\}$\;
                
%                 \STATE $\text{bonus}_{h}^k(\cdot, \cdot) \leftarrow \beta\left[ \phib{\cdot, \cdot}^\top \left(\Lambtil\ii{k}{h}\right)^{-1}\phib{\cdot, \cdot}   \right]^{1/2}$
                
%                 % \STATE $Q\ii{k}{h}(\cdot,\cdot) \leftarrow  \beta\left[ \phib{\cdot, \cdot}^\top \left(\Lambtil\ii{k}{h}\right)^{-1}\phib{\cdot, \cdot}   \right]^{1/2} + \quad \vdot{\w\ii{k}{h}, \phib{\cdot, \cdot}}$\;
                
%                 \STATE $Q\ii{k}{h}(\cdot, \cdot) \leftarrow \min \left \{ 
%                  \vdot{\w\ii{k}{h}, \phib{\cdot, \cdot}}
%                  + \text{bonus}_{h}^k(\cdot, \cdot)
%                 , H \right \}$
                 
%                 \STATE Update $\tilde{k}_h \leftarrow k$ \algorithmicand $\switchcountvar \leftarrow \switchcountvar + 1$
%             % }
%             % \Else{
%             %     $\ytil_h^k = 0$ \\
%             % }
%         % }
%         \ENDIF
%         \ENDFOR
    
    
%         %% Play Episode
%     % \STATE Observe initial state $x^k_1$\\
%     \FOR{step $h=1\ldots, H$}
%         \STATE Observe $x_h^k$.
%         \STATE take action $a\ii{k}{h} \leftarrow \argmax_{a\in \cA} Q\ii{\tilde{k}_h}{h}\left(x\ii{k}{h}, a\right)$, and get reward $r_{h}^k \leftarrow r_h(x_h^k, a_h^k)$ .
%         %
        
%         %
%          \STATE $\LambdaMAT\ii{k+1}{h} \leftarrow \LambdaMAT\ii{k}{h}  +  \phi\pp{x\ii{k}{h}, a\ii{k}{h}}\phi\pp{x\ii{k}{h}, a\ii{k}{h}}^\top$.
%          %
%          \STATE Update $\cC_h{\pp{\frac{\rho}{2H}}}$ with $ \phi\pp{x\ii{k}{h}, a\ii{k}{h}}\phi\pp{x\ii{k}{h}, a\ii{k}{h}}^\top$ and output $\M_h^{k+1}$.
%          %
%         \STATE $\Lambtil\ii{k+1}{h} \leftarrow \LambdaMAT\ii{k+1}{h}   + \M\ii{k+1}{h} $.
%     \ENDFOR
    
%     \ENDFOR
%     %%%%%%%
% \caption{Private LSVI-UCB}\label{alg:privrl}
% \end{algorithmic}
% \end{algorithm}

\begin{algorithm}[H]
\begin{algorithmic}[1]
% \SetAlgoLined
% \textbf{Input:} \\
% \STATE \textbf{Parameters: } 
\INPUT Privacy parameter $\rho$, policy update rate $C$, fail probability $p$, confidence width $\beta$.
% Let $M\ii{t}{h} \in \mathbb{R}^{d\times d}$ be the noise from the $\BM$ at episode $t$ for Gram matrix $\Lambda\ii{t}{h}$. \\

\STATE  $\binmechboundvar \defeq \binmechbound$

\STATE $\switchcostvar \defeq \switchingcost$ 
% \COMMENT{Max number of policy updates.}

\STATE  $\switchcountvar \leftarrow 1$\;

% \STATE  $\rho_0 \leftarrow \rho / (3 H^2 \switchcostvar)$
% \COMMENT{Gaussian mechanism privacy budget.}




\STATE For all $h\in[H]$,  let $\cC_h{\pp{\frac{\rho}{2H}}}$ be a private counter satisfying $\pp{\frac{\rho}{2H}}$-zCDP.  


\STATE 
% $\LambdaMAT\ii{1}{h} \leftarrow  2\binmechboundvar\I,\quad 
$\Lambtil_h^1 \leftarrow 2 \binmechboundvar \I$  for all $h\in[H]$\; 

\STATE  $\tilde{k} \leftarrow 1 $  for all $h\in[H]$
% \COMMENT{Last time the policy was updated.}

\FOR{$k=1, \dots, K$}
% {
    % % \dnedit{
    % \IF{ $\det\left(\Lambtil\ii{k}{h}\right) \geq C \det\left(\Lambtil\ii{\tilde{k}_h}{h}\right)$}
    % \STATE add here
    % \ENDIF
    % % }
        
        % \STATE Receive initial state $x_1^k$.
        % \FOR{$h = 1, \cdots, H$}
        % \STATE $\Lambda_h^{k+1} \leftarrow \Lambda_h^k + \phi(x_h^k,a_h^k) \phi(x_h^i, a_h^i)^\top $
        % \STATE Update $\cC_h \left( \frac{\rho}{2H} \right)$ with $\phi(x_h^k, a_h^k) \phi(x_h^k, a_h^k)^\top$ and output $\M_h^{k+1}$
        % \ENDFOR
        \IF{$\exists h \in [H], \det(\Lambtil_h^{k}) \geq C \det(\Lambtil_h^{\tilde{k}})$ \algorithmicand
            $\switchcountvar < \switchcostvar$} \label{lin:update}
        % \STATE $Q_{H+1}^k (\cdot,\cdot) \leftarrow 0$
        \FOR{$h = H, \cdots, 1$}
        % \STATE $\Lambtil_h^k \leftarrow 2\binmechboundvar \I + \sum_{i=1}^{k-1} \phi(x_h^i,a_h^i) \phi(x_h^i, a_h^i)^\top + \M_h^k $
        % \STATE Let $\widetilde{V}_{h+1}^k(x_{h+1}^i)
        % = \max_{a \in \cA} Q_{h+1}^{k} (x_{h+1}^i, a)$ for all $i\in[k-1]$.
        
        
        \STATE Let $V_i = r_h^i + \max_{a \in \cA} Q_{h+1}^{k} (x_{h+1}^i, a)$
        
         \STATE $\ytil_h^k \leftarrow \left(\sum_{i=1}^{k-1} \phi(x_h^i, a_h^i) 
         \left[ 
          r_h^i + \max_{a \in \cA} Q_{h+1}^{k} (x_{h+1}^i, a)
         \right]
         \right) + \etabf_h^k$, where $\etabf_h^k \sim \cN(0, \frac{6 H^2 \switchcostvar}{\rho})$
        
        % \STATE $\ytil_h^k \leftarrow \sum_{i=1}^{k-1} \phi(x_h^i, a_h^i) \left [r_h^i +  \widetilde{V}_{h+1}^k(x_{h+1}^i) \right] + \etabf_h^k$, where $\etabf_h^k \sim \cN(0, \frac{6 H^2 \switchcostvar}{\rho})$
        
        
        
        % \STATE $\ytil_h^k \leftarrow \y_h^k + \etabf_h^k$, where $\etabf_h^k \sim \cN(0, \frac{2H+2}{\rho_0})$
        \STATE $\w_h^k \leftarrow \left( \Lambtil_h^{k} \right)^{-1} \ytil_h^k$
        \STATE $\text{bonus}_h^k(\cdot,\cdot) \leftarrow \beta \left[ \phi(\cdot,\cdot)^\top \left( \Lambtil_h^k \right)^{-1} \phi(\cdot,\cdot) \right]^{1/2}$
        \STATE $Q_h^k(\cdot,\cdot) \leftarrow \min \{ \phi(\cdot,\cdot)^\top \w_h^k + \text{bonus}_h^k(\cdot,\cdot), H - h + 1 \}$
        \STATE Update $\tilde{k} \leftarrow k$ \algorithmicand $\switchcountvar \leftarrow \switchcountvar + 1$
        % \STATE $\pi_h^k(\cdot,\cdot) \leftarrow \argmax_{a \in \cA} Q_h^k (\cdot, a)$
        \ENDFOR
        % \ELSE
        % \STATE $Q_h^k \leftarrow Q_h^{k-1}, \pi_h^k \leftarrow \pi_h^{k-1}$, $\forall h \in [H]$
        \ENDIF
    
        %% Play Episode
    % \STATE Observe initial state $x^k_1$\\
    \FOR{step $h=1\ldots, H$}
        \STATE Observe $x_h^k$.
        \STATE Take action $a\ii{k}{h} \leftarrow \argmax_{a\in \cA} Q\ii{\tilde{k}}{h}\left(x\ii{k}{h}, a\right)$, and get reward $r_{h}^k \leftarrow r_h(x_h^k, a_h^k)$ .
        %
        
        % %
        %  \STATE $\LambdaMAT\ii{k+1}{h} \leftarrow \LambdaMAT\ii{k}{h}  +  \phi\pp{x\ii{k}{h}, a\ii{k}{h}}\phi\pp{x\ii{k}{h}, a\ii{k}{h}}^\top$.
        %  %
         \STATE Update $\cC_h{\pp{\frac{\rho}{2H}}}$ with $ \phi\pp{x\ii{k}{h}, a\ii{k}{h}}\phi\pp{x\ii{k}{h}, a\ii{k}{h}}^\top$ and output $\M_h^{k+1}$.
        %  %
        % \STATE $\Lambtil\ii{k+1}{h} \leftarrow \LambdaMAT\ii{k+1}{h}   + \M\ii{k+1}{h} $.
        \STATE $\Lambtil_h^{k+1} \leftarrow 2\binmechboundvar \I + \sum_{i=1}^{k} \phi(x_h^i,a_h^i) \phi(x_h^i, a_h^i)^\top + \M_h^{k+1} $
    \ENDFOR
    
    \ENDFOR
    %%%%%%%
\caption{Private LSVI-UCB}\label{alg:privrl}
\end{algorithmic}
\end{algorithm}



==> files/LinearRL/regret.tex <==
\subsection{Regret Analysis}\label{sec:regret}

After showing that \Cref{alg:privrl} is JDP, we finish the analysis by showing the regret guarantees.  

\begin{theorem}[Regret]\label{thm:regret}
For any $p\in (0,1)$, any privacy parameter $\rho>0$, if we set  $C = 2$ and $\beta=\betabound$ with $\chi = \chibound$ in \cref{alg:privrl}, then with probability $1-p$ , the total regret of Private LSVI-UCB (\cref{alg:privrl}) is at most 
\begin{align*}
    \mathrm{Regret}(K) \leq \regretbound
\end{align*}
By \Cref{lem:cdptodp}, \Cref{alg:privrl} satisfies $(\epsilon, \delta)$-differential privacy with $\epsilon = \rho + 2 \sqrt{\rho \log(1/\delta)}$. If $\epsilon < 1$, then the total regret of \Cref{alg:privrl} is at most
\begin{align*}
    \mathrm{Regret}(K)
    \leq \widetilde{O} \left ( d^{3/2} H^2 K^{1/2} + H^3 d^{5/4} K^{1/2} \pp{\log \left(\tfrac{1}{\delta} \right)}^2 \epsilon^{-1/2} \right)
\end{align*}
\end{theorem}

\dndelete{
We remark that in the bound above, the regret from injected perturbations to maintain privacy is of lower order compared to the non-private regret. We end up with a tighter dependency on $d$, while matching the non-private regret dependency on $H$ and $K$. }

\begin{proof}[Proof Sketch]
We present a proof sketch here for the regret analysis,  see \Cref{sec:regretfull} for full detail of the proof. Some steps are mostly similar to the ones in non-private setting \citet{jin2020provably}, there are several challenges we need to handle due to privacy noise. The regret proof follows the following steps:
 \begin{itemize}
    \item We condition on the events $\|\Lambtil_h^k - \LambdaMAT_h^k\| \leq \binmechboundvar$ and $\|\ytil_h^k - \y_h^k\| \leq \gaumechboundvar$, {which hold with high probability.}
     \item Construct new confidence bounds given the private statistics and show that the action-value function from \cref{alg:privrl} is optimistic.
    %  The perturbations added in $\Lambtil_h^{k}$ and $\ytil_h^{k}$ inflates the width of confidence bound. 
     \item Given the new confidence bounds, we follow similar steps  as in \citet{jin2020provably} and \citet{wang2021provably}.
 \end{itemize}

Note that on episode $k$, the agent acts according to policy $\pi_k$ which is given by  $\pi_{k}(x,h) = \argmax_{a} Q_h^{\tilde{k}}(x,a)$, where  $\tilde{k} \leq k$ be the
last episode the algorithm updated its policy for time step $h$.

\paragraph{Upper Confidence Bounds (UCB)} In this section fix any $h\in[H]$ and let $k\in[K]$ be an update episode for time step $h$ such that $\tilde{k} = k$. 

As described before, \cref{alg:privrl} uses a Least-Squares-Value-Iteration to estimate the action-value function $Q_h^{\star} \defeq \vdot{\phi(x,a), \w_h^{\star}}$, which is a linear function of the feature vectors.
%
The LSVI solution on episode $k$ and time-step $h$ is given by $\w_h^{k} = \pp{\Lambtil_h^k}^{-1} \ytil_h^k$, is an unbiased approximation to the true action-value function $Q_h^\star(x,a)$, as was shown in \citet{jin2020provably}. Furthermore, to achieve low regret the algorithm builds an optimistic action-value function $Q_h^k(x,a) = \vdot{\phi(x,a), \w_h^k} + \beta\sqrt{\phi(x,a)^\top\pp{\Lambtil_h^k}^{-1}\phi(x,a)}$, and follows a greedy policy $\pi_h^k(x) =\argmax_a Q_h^k(x,a)$.
The term $\beta$ is the confidence bound of the LSVI estimate, and has an effect on the final regret. 

% The optimistic action-value function,
% a bonus term in the form $\beta\sqrt{\phi(x,a)^\top\pp{\Lambtil_h^k}^{-1}\phi(x,a)}$, and set the action-value function $Q_h^k(x,a) = \vdot{\phi(x,a), \w_h^k} + \beta\sqrt{\phi(x,a)^\top\pp{\Lambtil_h^k}^{-1}\phi(x,a)}$.

In this section we show how to choose the confidence $\beta$ that ensures $Q_h^k$ is an optimistic function (i.e., $Q_h^k(x,a)\geq Q_h^\star(x,a)$ for all $(x,a)$), given the noise added to privatize the statistics. Let $\widehat{Q}_h^k(x,a) = \vdot{\phi(x,a), \w_h^{k}}$ be the private empirical action-value function maintained by \cref{alg:privrl} without the bonus term and $Q_h^\star(x,a)=\vdot{\phi(x,a), \w_h^{\star}}$ be the action-value function for the optimal policy $\pistar$. We want to find a $\beta$, such that for all $x,a\in \cS \times \cA$, we have $\left|\widehat{Q}_h^k(x,a)-{Q}_h^\star(x,a)\right|\leq  \beta\sqrt{\phi(x,a)^\top\pp{\Lambtil_h^k}^{-1}\phi(x,a)}$. 
%
%
%
We begin by decomposing the term $ \w_h^{k} - \w_h^\pi$ as follows:
\begin{align*}
        \w^{k}_h - \w^{\star}_h
     =\underbrace{ \pp{\Lambtil_h^{k}}^{-1} \pp{ \y_h^k} - \w^{\star}_h}_{\va}
     + \underbrace{\pp{\Lambtil_h^{k}}^{-1} \etabf_h^{k}}_{\vb} 
\end{align*}
%
%
Now we can write
$\widehat{Q}_h^k(x,a)-{Q}_h^\star(x,a)= \vdot{\phi(x,a), \va + \vb}$ and treat each term $\vdot{\phi(x,a), \va }$,  $\vdot{\phi(x,a), \vb}$ independently.
%
%
% Let $\binmechboundvar$ be the minimum eigenvalue of the matrix $\Lambtil_h^{\tilde{k}}$. 
%
%
Then, similarly as in  Lemma B.4 in \cite{jin2020provably} we give a confidence bound for the first term $\vdot{\phi(x,a), \va}$, which depends on the square root of the minimum eigenvalue of the Gram matrix $\Lambtil_h^{k}$:

\begin{align*}
\left|
    \vdot{\phi(x,a), \va} - \zeta_{h+1}
    %\bbP_h\pp{\tilde{\V}_{h+1}^{\tilde{k}} - \V_{h+1}^\pi}(x,a)
    \right| 
    \leq 
    \beta_0\sqrt{\phi(x,a)^\top ({\Lambtil_h^{k})^{-1}\phi(x,a)}}
\end{align*}
for $\beta_0 = \dndelete{16} \dnedit{5} H \sqrt{d\binmechboundvar\log(\chi)} + 6dH \sqrt{\log(\chi)} $ and $\zeta_{h+1}$ is a term that we analyze in detail in the appendix, for now we can set $\zeta_{h+1} = 0$.  It remains to give a confidence bound for the second term $\vdot{\phi(x,a), \vb}$. We have:

\begin{align}
    |\vdot{\phi(x,a), \vb}|
    % &\leq \nn{\etabf_h^{\tilde{k}}}_{(\Lambtil_h^{\tilde{k}})^{-1}}\sqrt{\phi(x,a)^\top (\Lambtil_h^{\tilde{k}})^{-1}\phi(x,a)} \\
    %
    \label{lin:phidotb:I}
    &\leq \frac{\nn{\etabf_h^{k}}}{\sqrt{ \binmechboundvar}} \sqrt{\phi(x,a)^\top (\Lambtil_h^{k})^{-1}\phi(x,a)} \\
    %
    \label{lin:phidotb:II}
    &\leq \frac{\lambtil_{y}}{ \sqrt{\binmechboundvar}}   \sqrt{\phi(x,a)^\top (\Lambtil_h^{k})^{-1}\phi(x,a)} 
\end{align}

The first inequality \eqref{lin:phidotb:I} follows because $\binmechboundvar$ is the minimum eigenvalue of $\Lambtil_h^{{k}\dndelete{_h}}$. The second inequality \eqref{lin:phidotb:II} follows because, with high probability, the norm on the Gaussian mechanism is $\nn{\etabf_h^{k}} \leq \gaumechboundvar$ for all $k,h\in[K]\times [H]$. The next step is to bound the ratio $ \frac{\lambtil_{y}}{ \sqrt{\binmechboundvar}}$.
Recall that $\gaumechboundvar \approx d H^2 \log(K) \rho ^{-1/2}$ and $\binmechboundvar \approx d^{1/2} \log(K) \rho^{-1/2}$, then we have:  
\begin{align}\label{eq:ratio}
    \frac{\gaumechboundvar}{ \sqrt{\binmechboundvar}}
    \leq
    %
    \frac{d H^2 }{{\rho}^{1/2}} \cdot 
    \frac{\rho^{1/4}}{d^{1/4}}  
=    \frac{d^{3/4} H^2 }{{\rho}^{1/4}} \defeq \beta_1
\end{align}
%
Notice that $\beta_1$ confidence bound is not a dominant term compared with $\beta_0$; thus, it does not contribute too much to the regret bound. The reason is that the noise added by the Gaussian mechanism is small thanks to the low switching cost of \cref{alg:privrl}. Finally, we can substitute $(\beta_0 + \beta_1)$ into the final confidence bound and get:
\begin{align*}
   \left |Q_h^k(x,a) - Q_h^\star(x,a) \right |
%   \left | \vdot{\phi(x,a), \va + \vb} \right | \\
    \leq 
    \pp{\beta_0 +  \beta_1 } \nn{\phi(x,a)}_{(\Lambtil_h^{k})^{-1}}
\end{align*}
Therefore, it suffices to set 
% $\beta =  17 H \sqrt{d\binmechboundvar\log(\chi)} + 6dH \sqrt{\log(\chi)} \geq 16 H  \sqrt{d\binmechboundvar\log(\chi)} + 6dH \sqrt{\log(\chi)} + H\sqrt{d \binmechboundvar} \rho^{-1/4}$
$\beta =  \betabound$ to satisfy the inequality.

\paragraph{Regret proof} 
In this section we use the following notation $\phi_h^k = \phi\pp{x_h^k, a_j^k}$.
Given our confidence bounds, the final steps in the regret analysis are similar to those in \citet{jin2020provably} and \citet{wang2021provably}.
First, by \cref{lem:B3}, \cref{lem:B4}, \cref{lem:B6} we have that with high probability, the regret of \cref{alg:privrl} is upper bounded by 
\begin{align}\label{eq:regretdecomposition}
     \text{Regret}(K) &\leq \sum_{k=1}^K \sum_{h=1}^H \tilde{\zeta}_h^k + 3 \beta \sum_{k=1}^K \sum_{h=1}^H \sqrt{(\phi_h^k)^\top \pp{\Lambtil_h^{\tilde{k}}}^{-1} \phi_h^k}
\end{align}
where  $\zeta_{h+1}^k$ is a zero-mean martingale difference sequence bounded by $2H$.  Thus, using standard concentration inequalities the first term from \cref{eq:regretdecomposition} is upper bounded by $2\sqrt{2 K H^3 \log(4/p)}$ with high probability. For the second term in \cref{eq:regretdecomposition}, by \cref{thm:switchingcost} we have that ${\phi_h^k}^\top (\Lambtil_h^{\tilde{k}})^{-1} \phi_h^k \leq 2 {\phi_h^k}^\top (\Lambtil_h^k)^{-1} \phi_h^k$ with high probability. Therefore, combining the last two inequalities and by the Cauchy-Schwarz inequality we get


% Then, conditioned on the high probability events that $\|\Lambtil_h^k - \LambdaMAT_{h}^k\|\leq \binmechboundvar$,  our update criteria in \Cref{alg:privrl} implies that ${\phi_h^k}^\top (\Lambtil_h^{\tilde{k}})^{-1} \phi_h^k \leq 2 {\phi_h^k}^\top (\Lambtil_h^k)^{-1} \phi_h^k$ for all $k\in[K]$. 
% to get $\sum_{k=1}^K \sqrt{(\phi_h^k)^\top {(\Lambtil_h^{\tilde{k}})}^{-1} \phi_h^k} \leq   \sqrt{K \sum_{k=1}^K(\phi_h^k)^\top \pp{\Lambtil_h^{\tilde{k}}}^{-1} \phi_h^k}$  
%
%
\begin{align*}
    % \text{Regret}(K) \leq \tilde{\delta}_h^k +  \Delta_h^{\tilde{k}} (x,a) 
    % \text{Regret}(K) \leq \sum_{k=1}^K \sum_{h=1}^H \tilde{\zeta}_h^{\tilde{k}} + 3 \beta \sum_{k=1}^K \sum_{h=1}^H \nn{\phi_h^k}_{(\Lambtil_h^{\tilde{k}})^{-1}}
    \text{Regret}(K)  &\leq 2\sqrt{2 K H^3 \log(3/p)} +  3 \beta H \sqrt{K \sum_{k=1}^K
    (\phi_h^k)^\top \pp{\Lambtil_h^{k}}^{-1} \phi_h^k}
    \label{eq:regret-decomp}
\end{align*}
%
%
% The second inequality follows from  applying Cauchy-Schwarz.  
The last step uses the trace-determinant lemma and elliptical potential lemma from \citet{abbasi2011improved}, and the fact that the minimum eigenvalue of $\Lambtil_h^k$ is $\binmechboundvar$. Thus we have 
\begin{align*}
    \text{Regret}(K)
    \leq 2\sqrt{2 K H^3 \log(3/p)} + 6 \beta H \sqrt{2dK \log \left( \frac{K + \binmechboundvar}{\binmechboundvar} \right)}
\end{align*}
% We can further write the upper bound on $\beta$ to be sum of a non-private term and a private term. The non-private component of $\beta$ scales with $dH$, and the private component scales with $H\sqrt{d \lambtil_\Lambda}$, where $\lambtil_\Lambda$ is a bound on the norm of the binary mechanism used to perturb $\Lambtil_h^{\tilde{k}}$. This is the key technical contribution in our regret guarantee proof. 
Finally, we can substitute $\beta = \betabound$ from the UCB analysis above and arrive at the final regret bound:
\begin{align*}
    \text{Regret}(K) \leq \regretbound
    % \widetilde{O} \left( d^{3/2} H^2 K^{1/2} + H^2 d^{5/4} K^{1/2} \rho^{-1/4} \right) 
\end{align*}
\end{proof}

==> files/LinearRL/switching_cost.tex <==

\subsection{Switching Cost}\label{sec:switchingcost}

We begin by analysing the switching cost of \cref{alg:privrl} since it will be used in the following \cref{sec:privacy} for the privacy analysis .

\input{files/theorems/swtichingcost_gao/theorem}
\input{files/theorems/swtichingcost_gao/proof_sketch}

The low switching cost guarantee above is crucial for our algorithm to achieve our improved regret guarantee. The main technique we use to reduce number of policy update is to check whether to update the policy at each episode. 
The criteria we use to signal policy changes is when determinant of the feature covariance matrix changes significantly. We use $\tilde{k}$ to denote the last episode index when we update the policy to be the one used in episode $k$. 

==> files/doubling.tex <==

\begingroup
\subsection{Doubling framework for tabular setting}
\newcommand{\IQ}{\check{Q}}
\newcommand{\IV}{\check{V}}
\newcommand{\Ir}{\check{r}}
\newcommand{\Ibeta}{\check{\beta}}

\begingroup
\newcommand{\trig}{\textrm{TRIGGERED}}
\begin{algorithm}[H]
\SetAlgoLined
\textbf{Parameters: } privacy parameter $\varepsilon$.
Let $n(s,a) \leftarrow 0$ $N(s,a) \leftarrow 0$ for all $s,a$\;
Let $\cL = \{2^{i-1} | 2^{i-1} \leq KH \} $ be a trigger set\;

\For{$k=1, \dots, K$}{
    %%%%%%%
    %% Play Episode
    Observe initial state $x_1^k$\\
    \For{step $h=1\ldots, H$}{
        take action $\aht = \argmax_{a} Q^k_h(\xht, a)$ and observe $x_{h+1}^k$. 
        Update $N(s,a) \leftarrow N(s,a) + 1$\;
        \If{$N(s,a) \in \cL$}{
            $n(s,a) = N(s,a)$\;
            Set $\trig = true$
        }
    }
    \eIf{$\trig $ is true}{
        Update $Q_h^{k+1}$ using $n(s,a)$\;
    }{
        $Q_h^{k+1} \leftarrow Q_h^{k}$ for all $h$\;
    }
}
\label{alg:doubling}
\caption{Doubling Framework for Tabular Setting}
\end{algorithm}
\endgroup
Let $n_k(s,a)$ denote the value used for computing $Q^k_h(s,a)$ for all $h\in [H]$.

Let $\cK$ be the set of episodes with no update. Let $h_0(k)$ be the first time an update is triggered in the $k$-th episode. Define the set $\cX_0 = \{ (k, h_0(k) ) | k\in \cK^C \}$ of events where the trigger happen for the first time in an episode. Also define the event set  $\cX = \{ (k, h ) |k\in\cK^C \text{ and } h_0(k) < h \leq H \}$ as the time steps where a trigger has happened in a previous round.
The 

Suppose we have a bound for $Q^k_h$ as 
\begin{align}\label{eq:bound}
    Q^k_h(s,a) \leq r(s, a) + P_{s,a} V^k_h + \beta(s,a)
\end{align}

Suppose $\beta^k_h(s,a) = \sqrt{\tfrac{w^k_h}{n_k(s,a)}}$.
Using the short-hand notation $I(k,h) = I\{ (k,h) \notin \cX \}$, the set $I(k,h)$ represents the events where the episode is not triggered or is the first round it gets triggered. Let $\IQ^k_h(s,a) = I(k,h)Q^k_h(s,a)$, $\Ir(s,a) = I(k,h)r(s,a)$ and $\Ibeta(s,a) = I(k,a)\beta(s,a)$. Then we can write the following inequalities: If $(k,h) \notin \cX_0$ then 
\begin{align}\label{eq:bound1}
    \IQ^k_h(s^k_h,a^k_h) \leq \Ir(s^k_h,a^k_h)  + P_{(s^k_h,a^k_h)}\IV^k_{h+1} + \Ibeta^k_h(s^k_h,a^k_h)
\end{align}
To show that \cref{eq:bound1} holds, consider two cases: if $(k,h) \in \cX$ then everything is zero. Otherwise the bound holds from \cref{eq:bound}. If $(k,h) \in \cX_0$ then we cannot do much so we use the trivial bound: 

\begin{align}\label{eq:bound2}
    \IQ^k_h(s^k_h,a^k_h) \leq \Ir(s^k_h,a^k_h)  + P_{(s^k_h,a^k_h)}\IV_{h+1}^k + \Ibeta^k_h(s^k_h,a^k_h) + 1
\end{align}

Skipping some steps, suppose that we can decomposed the regret as:

\begin{align*}
    \textrm{Regret}(K) \leq \sum_{k=1}^K\sum_{h=1}^H \Ibeta^k_h(s^k_h,a^k_h) + O(\sqrt{K})
\end{align*}


Let $i_{max} = \max\{i| 2^i \leq KH\}$.
Under the doubling framework, the Q function only changes once the amount of data doubles on any state/action pair. That is, the number of visits is always a multiple of 2 and can be written as $n_k(s,a) = 2^i$ for $i \leq i_{max}$. 
Recall that $\beta^k_h(s,a) = \sqrt{\tfrac{w^k_h}{n_k(s,a)}}$, thus the term $n_k(s,a)$ dictates how large the error is.
%
For any state/action pair and any $i\leq i_{max}$, we can bound the number of times $n_k(s,a) = 2^i$ using the following inequality:
\begin{align}
    \sum_{k=1}^K\sum_{h=1}^H   \bbI\{(s^k_h,a^k_h) = (s,a), n_k(s,a)=2^i \} \bbI\{(k,h)\notin \cX \} \leq 2^i
\end{align}

Let $\bbI(k,h, s, a, i) =  \bbI\{(s^k_h,a^k_h) = (s,a), n_k(s,a)=2^i \} \bbI\{(k,h)\notin \cX \}$.
Note that if $(k,h)\in \cX$ then the weight $w^k_h = 0$. Now we can decompose the sum $\sum_{k=1}^K\sum_{h=1}^H \Ibeta^k_h(s^k_h,a^k_h)$ using the indices $i=0,\ldots, i_{max}$:




\begin{align*}
    &\sum_{k=1}^K\sum_{h=1}^H \Ibeta^k_h(s^k_h,a^k_h) \\
    &= 
    \sum_{k=1}^K\sum_{h=1}^H  \sum_{s,a}\sum_{i=0}^{i_{max}}  \bbI\{(s^k_h,a^k_h) = (s,a), n_k(s,a) = 2^i \}\Ibeta^k_h(s,a)  \\ 
    &=
    \sum_{k=1}^K\sum_{h=1}^H  \sum_{s,a}\sum_{i=0}^{i_{max}}  \bbI\{(s^k_h,a^k_h) = (s,a), n_k(s,a) = 2^i \} \bbI\{(k,h)\notin \cX \}\sqrt{\tfrac{w^k_h}{n_k(s,a)}}  \\ 
    &=
    \sum_{k=1}^K\sum_{h=1}^H  \sum_{s,a}\sum_{i=0}^{i_{max}}  \bbI(k,h, s, a, i)\sqrt{\tfrac{w^k_h}{2^i}}  \\ 
   &=
    \sum_{s,a}\sum_{i=0}^{i_{max}} \sqrt{\tfrac{1}{2^i}}  \sum_{k=1}^K\sum_{h=1}^H  \bbI(k,h, s, a, i)\sqrt{w^k_h}  \\ 
      &=
    \sum_{s,a}\sum_{i=0}^{i_{max}} \sqrt{\tfrac{1}{2^i}}  \sum_{k=1}^K\sum_{h=1}^H  \sqrt{\bbI(k,h, s, a, i)}\sqrt{\bbI(k,h, s, a, i) w^k_h}  \\ 
          &=
    \sum_{s,a}\sum_{i=0}^{i_{max}} 
    \sqrt{\tfrac{1}{2^i}}
    \sqrt{ \sum_{k=1}^K\sum_{h=1}^H \bbI(k,h, s, a, i)}
    \sqrt{ \sum_{k=1}^K\sum_{h=1}^H \bbI(k,h, s, a, i) w^k_h}  \\ 
      &=
    \sum_{s,a}\sum_{i=0}^{i_{max}} 
    \sqrt{\tfrac{1}{2^i}}
    \sqrt{ \sum_{k=1}^K\sum_{h=1}^H \bbI(k,h, s, a, i)}
    \sqrt{ \sum_{k=1}^K\sum_{h=1}^H \bbI(k,h, s, a, i) w^k_h}  \\ 
         &\leq 
    \sum_{s,a}\sum_{i=0}^{i_{max}} 
    \sqrt{ 1}
    \sqrt{ \sum_{k=1}^K\sum_{h=1}^H \bbI(k,h, s, a, i) w^k_h}  \\
          &\leq 
    \sqrt{\sum_{s,a}\sum_{i=0}^{i_{max}}  1}
    \sqrt{ \sum_{s,a}\sum_{i=0}^{i_{max}}  \sum_{k=1}^K\sum_{h=1}^H \bbI(k,h, s, a, i) w^k_h}  \\
              &= 
    \sqrt{SA i_{max}}
    \sqrt{ \sum_{k=1}^K\sum_{h=1}^H w^k_h}  \\
\end{align*}


%%% End doubling section
\endgroup


\subsection{Doubling framework in Linear MDP Setting}
\begingroup
\newcommand{\vhat}{\widehat{\textbf{v}}}
\newcommand{\vecbf}{\textbf{v}}

\newcommand{\Chat}{\widehat{\textbf{C}}}
\newcommand{\C}{\textbf{C}}
\newcommand{\uptI}{I_{\textrm{upt}}}
\newcommand{\maxI}{i_{\textrm{max}}}


Let $\{\phi^k_h\}_{k\in[K],h\in[H]}$ be the sequence of feature vectors and $\Lambda^k_h$ is the gram matrix on time $(k,h)$ such that:
\[
\Lambda^k_h = \sum_{\tau=1}^{k-1} \phi^\tau_h  (\phi^\tau_h)^\top
\]

From \cite{jin2020provably} the regret is bounded by: 
\begin{align}
   \textrm{Regret}(K)\leq \sum_{k=1}^K\sum^H_{h=1}\sqrt{ (\phi^k_h)^\top (\Lambda^k_h)^{-1}\phi^k_h} + (\text{Other terms}) 
\end{align}


\paragraph{Our goal} in this section is to bound the sum 
$ \left( \sum_{k=1}^K\sum^H_{h=1} (\phi^k_h)^\top (\Lambda^k_h)^{-1}\phi^k_h\right)$
while minimizing the total number of updates.
If we can do that the next step is to use Cauchy-Schwartz.
% Here is an algorithm for Linear MDPs using the doubling framework:
For a fixed $h$, let $B(K, h)$ be the sum up to episode $K$ of the $h$ terms when the algorithm updates it's policy on every episode. From \cite{jin2020provably} we have the following bound:
\[
B(K, h) = \sum_{k=1}^K (\phi^k_h)^\top (\Lambda^k_h)^{-1}\phi^k_h \leq 2\log\left[\frac{\det(\Lambda_h^{K+1})}{\det(\Lambda_h^{0})}\right]
\]

We want to consider an algorithm that only updates it's policy when the number of observations doubles. Let $\uptI = \{2^1, 2^2, \ldots, 2^{\maxI}\}$ be the episode indices where we update the policy, where $\maxI < \log(K)-1$. In other words, the algorithm updates its policy $\log(K)$ times. Suppose the algorithm updates the policy ( $\w_h$ and $\Lambda_h$) on indices $\uptI$, then denote $B^2(K, h)$ as the bonus error under the doubling framework up to episode $K$ as
%
\begin{align*}
B^2(K, h) =   \sum_{i=0}^{\maxI} \sum_{k=2^i}^{2^{i+1}}  (\phi^k_h )^\top \left(\Lambda^{2^i}_h\right)^{-1} \phi^k_h
\end{align*}

Can we provide a similar bound here?
% %%%%%%%%
% %% Private Algorithm
% %%%%%%%%
% \begin{algorithm}[h]
% \SetAlgoLined
% % \textbf{Input:} \\
% \textbf{Parameters: } \;

% Initialize $\Lambhat^1_h = \lambda I $ and $\Lambda^1_h = \lambda I $ for all $h\in[H]$ \;
% Let $\cH = \emptyset$\tcp*{Feature vector history.}
% \For{$k=1, \dots, K$}{
%      \For{$h=H\ldots, 1$}{
%         \label{algolin:update}
%         $\w_h \leftarrow (\Lambda^k_h)^{-1} \sum_{\tau=1}^{k-1}\phib{\xht,\aht} \left( r_h(\xht,\aht) + \max_{a}  \w_{h+1}^\top \phib{\xht, a}  \right)$\\
%         $Q_h(\cdot,\cdot) = \min\left\{ \w_h^\top \phib{\cdot, \cdot} + \beta\left[ \phib{\cdot, \cdot}^\top (\Lambda^k_h )^{-1}\phib{\cdot, \cdot}   \right]^{1/2}, H \right\}$
%     }
    
%     %%%%%%%
%     %% Play Episode
%     Observe initial state $x_1^k$\;
%     \For{step $h=1\ldots, H$}{
%         Take action $\aht = \argmax_{a} Q_h(\xht, a)$ and observe $x_{h+1}^k$\;
%         $\Lambhat^{k+1}_h \leftarrow  \Lambhat^{k}_{h} + \phib{\xht,\aht} \phib{\xht,\aht}^\top$\;
%         Add to history: $\cH = \cH \cup \{ \phib{\xht,\aht} \}$\;
%         % Let $\lambhat_1, \ldots, \lambhat_d$ be the eigenvalues of $\Lambhat^{k+1}_h $\;
%         Let $\vhat_1, \ldots, \vhat_d$ be the eigenvectors of $\Lambhat^{k+1}_h $\;
        
%         Let $\Chat_1, \ldots, \Chat_d$ be a clustering of the feature vectors in $\cH$ based on proximity to the eigenvectors $\vhat_1, \ldots, \vhat_d$. That is,:
%         \[
%         \Chat_i = \{ \phi \in \cH | \forall_{\phi' \in \cH} \quad \vhat_i^\top \phi \leq \vhat_i^\top \phi' \}
%         \]
%         \For{$i = 1,\dots, d$}{
%             \If{$|\Chat_i| = 2|\C_i|$}{
%                 Update TRIGGER = True:\;
%                 $\C_i = \Chat_i$\;
%             }
%         }
%     }
% }
% \label{alg:doubling}
% \caption{Private LSVI-UCB}
% \end{algorithm}

\endgroup

==> files/lemmas/gaussian_adaptive/proof.tex <==

\begin{proof}
\gv{Explain adversary here:} 

In \Cref{alg:privrl}, we maintain bounded joint sensitivity .. 
\gv{Replace $n$ with $K$ everywhere.}
For a fixed bit $b\in \{0,1\}$, we abuse the notation by writing $V^b_i$ the distribution over possible outcomes for the $i$-th query, and $v_{\leq i}$ as the view of all realized outcome up to and including the $i$-th query. 


Hence, we can write the dependencies of the $i$-th query's distribution as $V^b_i(v_i | v_{\leq i - 1})$, where $v_{\leq i - 1}$ is the view of all realized output up to and including the $i$-th query. Similarly, we can write the joint distribution over possible views as $V^b(v_{\leq K})$. The budget of the $i$-th query, $\rho_i$, depends only on all queries up to the previous one. We explicitly show this dependency by writing the privacy budget as $\rho_i (v_{\leq i-1})$. 


We start by writing the integral for $\rho-$zCDP as:
\begin{align*}
     &\quad e^{(\alpha - 1)D_{\alpha}(V^0 \| V^1)}\\
     &= \int_{\mathcal{R}_1, \cdots, \mathcal{R}_K} (V^0 (v_{\leq K}))^{ \alpha} (V^1 (v_{\leq K}))^{1- \alpha}  dv_1 \dots dv_n\\
     &= \int_{\mathcal{R}_1} (V^0_1(v_1))^{\alpha} (V^1_1(v_1))^{1-\alpha} \dots \int_{\mathcal{R}_K} (V^0_n (v_K | v_{\leq K-1}))^{\alpha} (V^1_K (v_K | v_{\leq K-1}))^{1-\alpha} dv_K \dots dv_1
\end{align*}
Shifting the focus to the inner most integral, we can rewrite it as: 
\begin{align*}
    %
    &\int_{\mathcal{R}_K} (V^0_K (v_K | v_{\leq K-1}))^{\alpha} (V^1_K (v_K | v_{\leq K-1}))^{1-\alpha} dv_K \\
    &= \quad \exp{ \left( (\alpha-1)D_\alpha\left(V^0_K (v_K | v_{\leq K-1})|(V^1_K (v_K | v_{\leq K-1})\right) \right)} 
    % =  \int_{\mathcal{R}_n} (V^0_n (v_n | v_{\leq n-1}))^{\alpha} (V^1_n (v_n | v_{\leq n-1}))^{1-\alpha} dv_n \\
    % &\leq e^{(\alpha - 1) \alpha \rho_n  (v_{\leq n-1})} \leq e^{(\alpha-1) \alpha (\rho - \sum_{i=1}^{n-1} \rho_i(v_{\leq i-1}))}
\end{align*}
Note that the variable $\ytil_K$ follows the normal distribution, therefore we can write  $V^0_K (\ytil_K | \ytil_{\leq K-1}) = \cN(\y_K^0, \sigma^2 \I)$, where $\y_K^b$ is the statistic given user sequence $D_K^b$.
%
Then we can use a lemma from \cite{bun2016concentrated}
\begin{lemma}[Lemma 2.4 in \cite{bun2016concentrated}]
Let $\mu, \nu, \sigma\in \mathbb{R}$ and $\alpha \in [1, \infty)$. Then 
\begin{align*}
    \text{D}_\alpha(\cN(\mu, \sigma^2) \parallel \cN(\nu, \sigma^2))  = \frac{\alpha (\mu - \nu)^2}{2\sigma^2}
\end{align*}
\end{lemma}

Then 
\begin{align*}
 \quad \exp{\left( (\alpha-1)D_\alpha\left(V^0_K (v_K | v_{\leq K-1})|(V^1_K (v_K | v_{\leq K-1})\right) \right)} 
 = \exp\left({(\alpha-1) \frac{\alpha \|\y_K^0 - \y_K^1 \|^2}{2\sigma^2}}\right)
\end{align*}


We can substitute this expression in the original integral, and follow through 
\begin{align*}
    &\quad \exp\left({(\alpha - 1) D_{\alpha} (V^0 \| V^1)}\right) \\
    &=
    \int_{\mathcal{R}_1} (V^0_1(v_1))^{\alpha} (V^1_1(v_1))^{1-\alpha} \dots \int_{\mathcal{R}_n} (V^0_K (v_K | v_{\leq K-1}))^{\alpha} (V^1_K (v_K | v_{\leq K-1}))^{1-\alpha} dv_K \dots dv_1 \\ 
    &= \int_{\mathcal{R}_1} (V^0_1(v_1))^{\alpha} (V^1_1(v_1))^{1-\alpha} \dots
    %
    \exp\left({(\alpha-1) \frac{\alpha \|\y_K^0 - \y_K^1 \|^2}{2\sigma^2}}\right)
    dv_{K-1} \dots dv_1 \\ 
    %
    \vdots \\ 
    &=\prod_{i=1}^K \exp\left({(\alpha-1) \alpha \frac{\|y_i^0 - y_i^1 \|_2^2}{2\sigma^2}}\right) \\
    &=\exp\left({(\alpha-1) \alpha \frac{\sum_{i=1}^K\|y_i^0 - y_i^1 \|_2^2}{2\sigma^2}}\right)
\end{align*}
% \begin{align*}
%     &\quad e^{(\alpha - 1) D_{\alpha} (V^0 \| V^1)} \\
%     &\leq \int_{\mathcal{R}_1} (V^0_1 (v_1))^{\alpha} (V^1_1 (v_1))^{1-\alpha} \dots \int_{\mathcal{R}_{n-2}}(V^0_{n-2} (v_{n-2} | v_{\leq n-3}))^\alpha (V^1_{n-2} (v_{n-2} | v_{\leq n-3}))^{1-\alpha} \\
%     &\quad \left \{ e^{(\alpha - 1)  \alpha(\rho - \sum_{i=1}^{n-1} \rho_i (v_{\leq i-1}))} \int_{\mathcal{R}_{n-1}} (V^0_{n-1} (v_{n-1} | v_{\leq n-2}))^{\alpha} (V^1_{n-1}(v_{n-1} | v_{\leq n-2}))^{1-\alpha} dv_{n-1} \right \} dv_{n-2} \dots dv_1\\
%     &\leq \int_{\mathcal{R}_1} (V^0_1(v_1) )^{\alpha} (V^1_1(v_1) )^{1- \alpha} \dots \int_{\mathcal{R}_{n-2}}(V^0_{n-2} (v_{n-2} | v_{\leq n-3}))^{\alpha} (V^1_{n-2} (v_{n-2} | v_{n-3}))^{1-\alpha} \\
%     &\quad \left \{ e^{(\alpha - 1)\alpha(\rho  - \sum_{i=1}^{n-1} \rho_i (v_{\leq i - 1}))} e^{(\alpha - 1) \alpha \rho_{n-1} (v_{\leq n-2})} \right \} dv_{n-2} \dots dv_1\\
%     &= \int_{\mathcal{R}_1} (V^0_1 (v_1))^{\alpha} (V^1_1(v_1))^{1-\alpha} \dots \int_{\mathcal{R}_{n-2}} (V^0_{n-2} (v_{n-2} | v_{\leq n-3}))^{\alpha} (V^1_{n-2} (v_{n-2} | v_{\leq n-3}))^{1-\alpha} \\
%     &\quad \left \{ e^{(\alpha - 1)\alpha(\rho  - \sum_{i=1}^{n-2} \rho_i (v_{\leq i-1}))} \right \} d v_{n-2} \dots  dv_{1}\\
%     &\leq e^{(\alpha - 1)\alpha \rho  }  
% \end{align*}

By \cref{thm:switchingcost}, the algorithm chooses $y_i^0 \neq y_i^1$ at most $dH\log(K)$ times. 
% The following \Cref{lem:sensitivity} gives the $\ell_2$-sensitivity 

Therefore by \cref{lem:sensitivity} we have that $\|y_i^0 - y_i^1 \|_2^2\leq 2 H +2$, therefore it follows that $\sum_{i=1}^K\|y_i^0 - y_i^1 \|_2^2\leq d H (2H + 2)\log(K)$.

From \cref{alg:privrl} we have that $\sigma^2 = \frac{2H(2H + 2)d\log(K)}{\rho}$.

\begin{align*}
    \exp\left({(\alpha - 1) D_{\alpha} (V^0 \| V^1)}\right)
    \leq \exp\left((\alpha - 1) \alpha \rho\right)
\end{align*}
\end{proof}

==> files/lemmas/gaussianmatrix/lemma.tex <==
\begin{lemma}[Gaussian Matrix Mechanism]
Suppose we have a dataset $X =\{ \x_1, \ldots, \x_n\}$, where each $\x_i\in \mathbb{R}^d$ is a $d$-dimensional vector with bounded $\ell_2$-norm such that: $\|\x_i\|_2\leq L$ for all $i\in [n]$. 
Consider releasing the following statistic privately: $\V = \sum_{i=1}^n \x_i\x_i^\top$, where each $\x_i\x_i^\top$ alters the Frobenius norm by at most $L^2$.
%
The Gaussian Matrix Mechanism samples the noise matrix $\Z'$, where $\Z'\in\mathbb{R}^{d\times d}$ is a random matrix where each entry $\Z'_{i,j} \sim  \cN\pp{0, \frac{L^4}{2\rho}}$ i.i.d, gets the symmetric matrix $\Z = (\Z' + {\Z'}^{\top})/\sqrt{2}$ and outputs:
%
\begin{align*}
    \cM_G(X) = \sum_{i=1}^n \x_i\x_i^\top + \Z
\end{align*}
%
Then $\cM_G$ satisfies ${\rho}$-zCDP and is $\pp{\frac{L^2\pp{4\sqrt{d+1} + 2\ln(2/\beta)}}{\sqrt{2\rho}}, \beta}$-$\ell_2$-accurate.
% $\pp{L^2\sqrt{\frac{}{2\rho}} \pp{4\sqrt{d+1} + 2\ln(2/\beta)}, \beta}$-$\ell_2$-accurate.
\end{lemma}

==> files/lemmas/gbmm/lemma.tex <==
\begin{lemma}[Gaussian Binary Matrix Mechanism (GBMM)]
\gv{GV: Will remove or update this. }
Let $\cC$ be a binary mechanism private counter initialized with parameter $\rho$.




The GBMM takes as input a stream of $d$-dimensional vectors $ \x_1, \ldots, \x_K$ over a sequence of $K$ episodes.



On each episode $k\in [K]$, the goal is to release the following statistic $\V_k = \sum_{i=1}^k \x_i\x_i^\top$. Note that $\|\x_i\x_i^\top\|_2\leq L^2$.
%
On episode $k$, the GBMM releases $\V_k + \mH_k$, where $\mH_k$ is the sum of at most $\log(T=HK)$ Gaussian noise matrices with parameter $\log(K)L^4/\rho$.
Then, GBMM satisfies $\rho$-zCDP and  $\| \mH_k \|_2 \leq \frac{L^2\log(K) \pp{4\sqrt{d+1} + 2\ln(2/\beta)} }{\sqrt{2\rho}}$
\end{lemma} 


\swcomment{can we not use $\x$? is this supposed to be a general result or specificially for our algo?}

% \begin{lemma}[Gaussian Binary Matrix Mechanism (GBMM)]
% Suppose we observe a stream of $d$-dimensional vectors $ \x_1, \ldots, \x_K$ over a sequence of $K$ episodes.Each $\x_i\in \mathbb{R}^d$ has bounded $\ell_2$-norm such that: $\|\x_i\|_2\leq L$ for all $i\in [n]$. On each episode $k\in [K]$, the goal is to release the following statistic $\V_k = \sum_{i=1}^k \x_i\x_i^\top$. Note that $\|\x_i\x_i^\top\|_2\leq L^2$.
% %
% On episode $k$, the GBMM releases $\V_k + \mH_k$, where $\mH_k$ is the sum of at most $\log(T=K)$ Gaussian noise matrices with parameter $\log(K)L^4/\rho$.
% Then, GBMM satisfies $\rho$-zCDP and  $\| \mH_k \|_2 \leq \frac{L^2\log(K) \pp{4\sqrt{d+1} + 2\ln(2/\beta)} }{\sqrt{2\rho}}$
% \end{lemma}

==> files/lemmas/swtchingcost_gao/det_inequality.tex <==
\begin{lemma}
Assume $m \leq n$, $A = \M_m + 2\binmechboundvar \I + \sum_{i=1}^m \phi_i \phi_i^\top $, $B = \M_n + 2\binmechboundvar \I + \sum_{i=1}^n \phi_i \phi_i^\top $. Then, if $A^{-1} \npreceq 2B^{-1}$, we have
\begin{equation*}
    \log \det B \geq \log \det A + \log 2
\end{equation*}
\label{lem:L2-switchingcost}
\end{lemma}


==> files/lemmas/swtchingcost_gao/det_inequality_proof.tex <==

First, we state the following two linear algebra facts that will be used in the proof:
\begin{fact}[Woodbury matrix identity] For any PSD matrices $A$, $\Delta \in \mathbb{R}^{d \times d}$. Suppose $A$ is invertible, then we have:
\begin{align*}
    (A + \Delta)^{-1} = A^{-1} - A^{-1} \Delta^{1/2}(\I + \Delta^{1/2} + A^{-1} \Delta^{1/2})^{-1} \Delta^{1/2} A^{-1}
\end{align*}
\end{fact}
\begin{fact}[Matrix determinant lemma] For any PSD matrices $A$, $\Delta \in \mathbb{R}^{d\times d}$, suppose $A$ is invertible, then 
\begin{equation*}
    \det(A + \Delta) = \det(\I + \Delta^{1/2} A^{-1} \Delta^{1/2}) \cdot \det(A)
\end{equation*}
\end{fact}

\begin{proof}
By the matrix determinant lemma, we only need to show that:
\begin{equation*}
    \lambda_{\max}(\I + \Delta^{1/2} A^{-1} \Delta^{1/2}) \geq 2
\end{equation*}
Since $A^{-1} \npreceq 2B^{-1}$, it must be the case that, for some $x$ with $\nn{x}_2 = 1$, and 
\begin{equation*}
    x^\top (A^{-1} -2B^{-1})x \geq 0 
\end{equation*}
Denote $\Delta = B - A \succ 0$. By Woodbury identity, we have:
\begin{align*}
    &\quad x^\top (A^{-1} - 2B^{-1})x \\
    &= x^\top (2 A^{-1} \Delta^{1/2}(\I + \Delta^{1/2} A^{-1} \Delta^{1/2})^{-1} \Delta^{1/2} A^{-1} - A^{-1})x\\
    &\geq 0
\end{align*}
Let $y = A^{-1/2}x$, we then have,
\begin{align*}
    &\quad 2y^\top A^{-1/2} \Delta^{1/2} (\I + \Delta^{1/2} A^{-1} \Delta^{1/2})^{-1} \Delta^{1/2} A^{-1/2} y\\
    &\geq \nn{y}_2^2
\end{align*}
Hence, 
\begin{equation*}
    \lambda_{\max} (A^{-1/2} \Delta^{1/2} (\I + \Delta^{1/2} A^{-1} \Delta^{1/2})^{-1} \Delta^{1/2} A^{-1/2}) \geq 1/2
\end{equation*}
Let us denote $C = A^{-1/2}\Delta^{1/2}$, we have:
\begin{equation*}
    \lambda_{\max} (C (\I + C^\top C)^{-1} C^\top) \geq 1/2
\end{equation*}
Let $C = U \Sigma V^\top$ be the SVD decomposition of $C$, where $U$ and $V$ are orthogonal and $\Sigma$ is diagonal. Then we have,
\begin{align*}
    &\quad C(\I + C^\top C )^{-1} C^\top\\
    &= U \Sigma V^\top (\I + V \Sigma^2 V^\top)^{-1} V \Sigma U^\top\\
    &= U \Sigma (\I + \Sigma^2)^{-1} \Sigma U^\top
\end{align*}
Note that $\Sigma = \mathrm{diag}(\sigma_1, \sigma_2, \dots, \sigma_d)$ is diagonal, we have
\begin{equation*}
    \max_i \frac{\sigma_i^2}{1 + \sigma_i^2} \geq 1/2 \Rightarrow \max_i \sigma_i^2 \geq 1
\end{equation*}
we additionally write $\I + \Delta^{1/2} A^{-1} \Delta^{1/2}$ as 
\begin{equation*}
    \I + \Delta^{1/2} A^{-1} \Delta^{1/2} = \I + C^\top C = \I + V \Sigma^2 V^\top
\end{equation*}
Thus we have
\begin{equation*}
    \lambda_{\max}(\I + \Delta^{1/2} A^{-1} \Delta^{1/2}) \geq 2
\end{equation*}
as desired. 
\end{proof}

==> files/lemmas/swtchingcost_gao/potential_upper_bound.tex <==
\begin{lemma}[Adapted from Lemma 1 in \cite{gao2021provably}]
\label{lem:potentialupperGao}

Let $\phi_i$ are $d-$dimensional vectors satisfying $\nn{\phi_i} \leq 1$. For any $K>0$, let $\A = 2\binmechboundvar \I  + \M_K+ \sum_{i=1}^K \phi_i \phi_i^\top$.
On the event that $\nn{\M_K} \leq \binmechboundvar $, we have
\begin{equation*}
    % \log \det A = O(d \log K)
    \log \det (\A) = d\log\left( d(K + \binmechboundvar) \right)
\end{equation*}
\end{lemma}

==> files/lemmas/swtchingcost_gao/potential_upper_bound_proof.tex <==
\begin{proof}{of \cref{lem:potentialupperGao}.}
Assume $\phi_i^d = (\alpha_1, \alpha_2, \dots, \alpha_d)^\top$. Since $\nn{\phi}_2^2 \leq 1$, we know that $|\alpha_i| \leq 1$ for all $i \in [d]$. Since $\phi_i^d (\phi_i^d)^\top = (\alpha_i \alpha_j)_{ij}$, the absolute value of each component of $\phi_i^d (\phi_i^d)^\top$ is no more than $1$.
Similarly, on the event that $\nn{\M_K}\leq \binmechboundvar $, we know that the absolute value of each component of $\M_K$ is not more than $\binmechboundvar$. Hence, the absolute value of each component of $\A$ is no more than $K + \binmechboundvar$. 

Use $\widetilde{\A}_d = (a_{ij})$ to denote a $d-$dimensional matrix satisfying the features above, i.e. $|a_{ij}| \leq K + 2\binmechboundvar$. Clearly, if the $1$st row and $j_\text{th}$ column are deleted, the rest $(d-1)$-dimensional matrix is $\widetilde{\A}_{d-1}$. Hence, we have:
\begin{align*}
    |\det(\tilde \A_d)| &\leq \sum_{j=1}^d |a_{1d}| \cdot |\det(\widetilde{\A}_{d-1})|\\
    &\leq d \cdot (K + \binmechboundvar) \cdot |\det(\widetilde{\A}_{d-1})|\\
    &\leq d^d (K + \binmechboundvar)^d
\end{align*}
Hence, we have $\log \det( \A )= d \log d + d\log(K + \binmechboundvar) = d\log\left( d(K + \binmechboundvar) \right)$
\end{proof}

==> files/old/FTPL.tex <==
\section{Follow the Perturbed Leader in Linear Bandits}

\paragraph{Idea}: Use \cref{lem:SwitchingCost} to give a Follow-The-Perturbed-Leader algorithm for linear bandits. Using the fact that the regret can be decomposed as:

\begin{lemma}[\cite{kalai2005efficient}]
Suppose the agent takes actions $\theta_1, \ldots, \theta_T$ and incurs losses $\ell_1(\theta_1), \ldots, \ell_T(\theta_T)$. If the agent chooses actions as:
\begin{align}\label{eq:FTPLopt}
    \theta_t = \argmin_{\theta} \pp{\sum_{i=1}^{t-1} \ell_i(\theta) + R(\theta)}
\end{align}
where $R(\cdot)$ is a regularization function. Then the regret is
\begin{align}\label{eq:FTPLexpectedRegret}
    \bbE{R_T} = \bbE{R(\theta_*)-R(\theta_1)} + \sum_{t=1}^T \bbE{ \ell_t(\theta_t) - \ell_t(\theta_{t+1})} 
\end{align}
where $\theta_* = \argmin_{\theta} \pp{\sum_{t=1}^{T} \ell_t(\theta) }$.
\end{lemma}

In the linear bandits setting, let $\cA_t$ be the context on time $t$.
We can set the loss function on time $t$ as:

\begin{align}
    \ell_t(\theta) = \vdot{\pp{\argmax_{a_t\in \cA_t}}, \theta_* } = -r_t
\end{align}

Using the switching cost lemma (\ref{lem:SwitchingCost}), if the loss functions are bounded then we can bound the second term of \cref{eq:FTPLexpectedRegret} as 
%
\begin{align*}
   \sum_{t=1}^T \bbE{ \ell_t(\theta_t) - \ell_t(\theta_{t+1})} \leq O\pp{d\log(T)} 
\end{align*}

Next we just need to bound $\bbE{R(\theta^*)-R(\theta_1)} $.

Note that if $R(\theta) = \lambda\nn{\theta}_1$, then the optimization \cref{eq:FTPLopt} corresponds to a ridge regression.

==> files/old/dp_low_switching_cost.tex <==
\section{Slowly Updating Linear Bandits}
\newcommand{\explore}{\mathrm{EXPLORE}}
\begin{algorithm} \caption{Slow Update Linear UCB}
\label{alg:slow-upd-ucb}
\SetKwInput{kwInit}{Initialize}
\SetKwInput{kwParam}{Parameters}
\kwParam{policy update rate $c$}
\kwInit{Gram matrix $V_0 \leftarrow \lambda I$ and $y_0 \leftarrow 0$}
\kwInit{previous update index $\tau = 0$ and update index $u=1$}

\For{each round $t = 1, \dots, T$}
{
\If{\upt}
{
Observe decision set $\mathcal{A}_t$.\\
Observe regularized $\Vtil_t \leftarrow \V_t + \mH_t$ and perturbed $\ytil = \cM_y(u)$\\
Compute regressor $\thetahat_t = \Vtil^{-1}_t \ytil_t$\\
Construct confidence set $C_t = \{ \theta: \| \theta - \thetatil_t \|_{\Vtil_t} \leq \sqrt{\beta_t} \}$ 

}
Pick action $\avec_t = \arg \max_{\avec \in \mathcal{A}_t} \langle \thetahat_\tau, \avec \rangle + \beta_\tau \| \avec \|_{\Vtil_\tau^{-1}}$\\
Play $\avec_t$ and observe reward $r_t$\\
Feed $\avec_t \avec_t^\top$ to $\cM_V$\\
Update $\Vtil_t \leftarrow \cM(t)$
}
\end{algorithm}
\begin{assumption}
\label{asmp: bounded-mean-reward}
We assume 
\begin{itemize}
    \item Bounded mean reward $|\langle \thetabf^*, \avec \rangle | \leq B$ with $B \geq 1$
\end{itemize}
\end{assumption}
\begin{assumption} 
\label{asmp: bounded-action}
For all rounds $t = 1, \dots, n$ and actions $\avec \in \mathcal{A}_t$, we assume
\begin{itemize}
    \item Bounded action set: $\|\avec \|_2 \leq L$
\end{itemize}
\end{assumption}
\begin{assumption}
\label{asmp: bounded-reward}
We assume 
\begin{itemize}
    \item Bounded reward vector $\|\thetabf^* \|_2 \leq S$
\end{itemize}
\end{assumption}
\begin{assumption} For all rounds $t = 1, \dots, n$, we assume
\begin{itemize} 
    \item The added noise by the binary mechanism $\mH_t$ is positive semidefinite {\color{red}this is no longer needed in our algorithm? }
\end{itemize}
\end{assumption}
\begin{assumption}
\label{asmp:reward-formula}
For all rounds $t = 1, \dots, n$, we assume:
\begin{itemize}
    \item $r_t = \langle \thetabf^*, \avec_t \rangle + \eta_t$ where $\eta_t$ is $\sigma^2-$conditionally subgaussian on previous actions and rewards
\end{itemize}
\end{assumption}
\begin{assumption} For all rounds $t = 1, \dots, n$, we assume the
\begin{itemize}  
    \item $\|\mH_t\| \leq \rho_{\max}$, $\|\mH_t^{-1}\| \leq 1/\rho_{\min}$, $\|\h_t\|_{\mH_t^{-1}}\leq \gamma$ 
\end{itemize}
\end{assumption}
\begin{proposition}
\label{prop:calc-beta}
Suppose Assumptions $\ref{asmp: bounded-reward}$ to $\ref{asmp:reward-formula}$ holds, and let $\rho_{\max}, \rho_{\min},$ and $\gamma$ be $(\alpha/2n)$-accurate for some $\alpha \in (0,1)$, and horizon $n$. Then $(\beta_t)_{t=1}^n$ is a $(\alpha, n)-$accurate where 
\begin{align*}
    \beta_t &= \sigma\sqrt{2\log(2/\alpha) + \log(\det(\V_t)) - d\log(\rho_{\min})} + S\sqrt{\rho_{\max}} + \gamma\\
    &\leq \sigma\sqrt{2\log(2/\alpha) + d\log\left( \frac{\rho_{\max}}{\rho_{\min}} + \frac{tL^2}{d \rho_{\min}}\right)} + S\sqrt{\rho_{\max}} + \gamma \tag{if Assumption \ref{asmp: bounded-action} also holds}
\end{align*}
\end{proposition}
\begin{theorem} (Regret of Algorithm \ref{alg:slow-upd-ucb})
Suppose Assumptions $\ref{asmp: bounded-mean-reward}$ to $\ref{asmp:reward-formula}$ hold and the $\beta_t$ are given by Proposition $\ref{prop:calc-beta}$. Then with probability at least $1 - \alpha$, the pseudo-regret of Algorithm $\ref{alg:slow-upd-ucb}$ is bounded by 
\begin{equation}
    \hat{R_n} \leq B\sqrt{8n}\left[ \sigma\left( 2\log\left( \frac{2}{\alpha}
    \right) + d\log \left(\frac{\rho_{\max}}{\rho_{\min}}\right)\right) \right]
\end{equation}
\end{theorem}

==> files/old/linear_bandits.tex <==
\section{Slowly Updating Linear Stochastic Bandits }\label{sec:linearbandits}
\begingroup
\newcommand{\Texp}{{T_0}}
\newcommand{\rhomax}{\rho_{\max}}
\newcommand{\rhomin}{\rho_{\min}}



\paragraph{Idea:}
\begin{itemize}
    \item Improve \cite{sheffet2017differentially} by having an exploration phase at the beginning.
    \item Also improve by doing slow updates.
\end{itemize}

\paragraph{Notation} At round $t$ the learner observes a decision set $\cA_t\subset \bbR$ and takes action $A_t \in \cA_t$. Then the reward is given by:
\begin{align*}
    r_t = \vdot{\theta_*, A_t} + \eta_t
\end{align*}
where $\eta_t$ is $1$-subgaussian given $A_1, r_1, \ldots, A_{t-1}, r_{t-1, A_{t-1}}$.
The pseudo-regret is given by
\begin{align*}
    \hat R_{t} = \sum_{i=1}^t \max_{a\in \cA_t} \vdot{\theta_*, a - A_t}
\end{align*}


\begin{assumption} We assume the following
\begin{enumerate}
    \item $\nn{a}_2 \leq L $ for all $a \in \cup \cA_t$.
\end{enumerate}
\end{assumption}

\begin{assumption}
for all $t$
\begin{itemize}
    \item $\|\mH_t\| \leq \rhomax$, $\|\mH_t^{-1}\| \leq 1/\rhomin$, $\|\h_t\|_{\mH_t^{-1}}\leq \gamma$ 
\end{itemize}
\end{assumption}


\begin{lemma}
Let $H_t$ 
\end{lemma}

\newcommand{\upt}{\mathrm{UPDATE}}
\newcommand{\explore}{\mathrm{EXPLORE}}

\begin{algorithm}[H]
\SetAlgoLined
% \textbf{Input:} \\
\textbf{Parameters: } privacy parameter $\varepsilon$, policy update rate $c$ \\
% Let $M\ii{t}{h} \in \mathbb{R}^{d\times d}$ be the noise from the $\BM$ at episode $t$ for Gram matrix $\Lambda\ii{t}{h}$. \\
$\tau=0 $ \tcp*{Last time the policy was updated.}
$u = 1$ \tcp*{Update index.}

% Let $\sigma = \sqrt{2\ln(1.25/\delta)} \frac{1}{\varepsilon}$\\


Initialize $d \times d$ dimensional private counter $\cM_V \leftarrow \BM(T,\sigma)$ \\
Initialize $d$ dimensional private counter $\cM_y \leftarrow \BM(T,\sigma)$ \\

% Let $\cE = \rho_{\max} \approx O(\frac{1}{\eps})$ \tcp*{Privacy error}
Note that $\rhomax \approx\frac{\sqrt{d}}{\eps}\log\log(T)$\\
Let $\widetilde{\rhomax} = \rhomax + \text{Lap}\pp{\tfrac{2}{\eps_1}}$ \tcp*{noisy threshold}
Let $\alpha = \frac{8\log(T) + \log(2/\beta)}{\eps_1}$ \tcp*{Sparse mechanism error}

Initialize $V_0 \leftarrow \lambda I$ and $\y_0 \leftarrow 0_\text{d}$ \\
Set $\explore \leftarrow \TRUE$\\
\For{$t=1, \dots, T$}{
    Set $\upt \leftarrow \FALSE$\\
    Observe decision set $\cA_t$. \\
    \uIf{$\explore$}{
        \If{$\DET{\V_t}/\DET{\V_0} + \mathrm{Lap}\pp{\tfrac{4}{\eps_1}} \leq \pp{\widetilde{\rhomax} + \alpha }$}{
           Set $\upt \leftarrow \TRUE$ 
        } 
    }\Else{
        Set $\explore \leftarrow \FALSE$\\
        \If{ $\det\pp{\Vtil_t} \geq c\det\pp{\Vtil_\tau}$}{
            Set $\upt \leftarrow \TRUE$ 
        }
    }
    
    \If{ $\upt$}{
        $u \leftarrow u + 1$\\
        Feed $\left(\sum_{i = \tau}^t \avec_i r_i\right)$ to $\cM_y$ 
            and get $\ytil_t = \cM_y(u)$ \\
        %
        Compute $\thetahat_{t-1} = \Vtil_{t-1}^{-1}  \ytil_{t-1}$ and construct confidence set $C_t = \left\{ \theta : \nn{\theta - \thetahat_{t-1}}_{\Vtil_{t-1}} \leq \sqrt{\beta_t} \right\}$ \\
        %
        % Let $\thetatil_t = \argmax_{\theta \in  C_{t}} \max_{\avec\in\cA_t} \vdot{\theta, \avec}$ \tcp*{Choose optimistic estimate.}
        Update $\tau=t$ \tcp*{update index}
    }
    // Let $\va_t,\thetatil_t =  \argmax_{\va\in\cA_t}\argmax_{\theta \in  C_{\tau}} \vdot{\theta, \avec}$\\ 
    % $\avec_t = \argmax_{\avec \in\cA_t } \vdot{\thetatil_\tau, \avec}$ \tcp*{choose best action.}
    $\va_t= \argmax_{\va \in \cA_t} \vdot{\thetahat_\tau, \va} + \beta_\tau \nn{\va}_{\Vtil_{\tau}^{-1}}$
    \tcp*{choose best action.}
    
    Play $\avec_t$ and observe reward $r_t$ \\
    %  Update $V_t = V_{t-1} + A_t A_t^\top$ and $y_t = y_{t-1} + A_t r_t$\tcp*{Update Gram matrix} 
     
    Feed $\avec_t \avec_t^\top$ to $\cM_V$ \\
    $\Vtil_t \leftarrow \cM_V(t)$\\
    % $\y_t \leftarrow \avec_t r_t$ \\
}   
\caption{Slowly Updating DP-UCB}\label{alg:lsb}
\end{algorithm}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Analysis} \label{sec:LSBanalysis}
Let $\va_1,\ldots, \va_T \in \pp{\cA_1\times,\ldots,\times\cA_T}$ be the sequence of actions by \cref{alg:lsb}. Let $\V_t = \sum_{i=1}^t \va_i\va_i^\top + \V_0$ and $\y_t = \sum_{i=1}^t \va_t r_t$.
%
For all $t\in[T]$ we have that $\Vtil_t \leftarrow \cM_v(t)$ is an approximate count of $\V_t$ where $\cM:[T]\rightarrow \bbR^{d\times d}$ is a binary mechanism with privacy parameter $\eps$. Let us write $\Vtil_t = \V_t + \mH_t$ such that $\mH_t$ is the noise added by the binary mechanism.
Likewise, let $\ytil_t = \y_t + \h_t$.

%%%%%%%%%%%%%%%%%%%%%%%%%
%% Begin: eward decomposition 
%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Prelim}

We can decompose the error as
\begin{align}
\notag
    \vdot{\thetabf^*, \va^*_t - \va_t} 
    \notag
    &= \vdot{\thetabf^*, \va^*_t}  - \vdot{\thetabf^*,  \va_t}  \\
    \notag
    &\leq \vdot{\thetatil_0, \va_t}  - \vdot{\thetabf^*,  \va_t}  \\
    \label{eq:rewardDecompositionI}
    &= \vdot{\thetatil_0 - \thetahat_0, \va_t}  + \vdot{\thetahat_0 - \thetabf^*,  \va_t} \leq 2S\nn{\va_t}  
    % &=  \vdot{\thetabf^* - \thetahat_0 + \thetahat_0, \va^*_t - \va_t}  \\ 
    % &= 
\end{align}

%% Lemma
\begin{lemma}[Lemma 11 in \cite{abbasi2011improved}]\label{lem:elipticalPotential}
Let $\va_1, \ldots \va_t$ be a sequence in $\bbR^d$, $\V_0$ a PSD matrix and define $\V_t = \V_0 + \sum_{i=1}^t \va_i \va_i^\top$. If $\nn{\va_i} \leq L$ and $\lambda_{\min} (\V) \geq \max(1,L^2)$ then
\begin{align*}
    \log\pp{\frac{\det( \V_t)}{\det(\V_0)}} \leq \sum_{i=1}^t \nn{\va_i}^2_{\V_{i-1}^{-1}}
    \leq 2 \log\pp{\frac{\det(\V_t)}{\det(\V_0)}} 
\end{align*}
\end{lemma}



%%%%%%%%%%%%%%%%%
%% Lemma
\begin{lemma}[Lemma 12 in \cite{abbasi2011improved}  ] \label{lem:normbound}
Let $A,B,C$ be PSD matrices such that $A = B+ C$. we have that 
\begin{align*}
    \sup_{x\neq 0}\frac{x^\top A x}{x^\top B x} \leq \frac{\det(A)}{\det(B)} 
\end{align*}
\end{lemma}


% \begin{lemma}
% If $\mH\in\mathbb{R}^{d\times d}$ is a matrix such that $\nn{\mH}\leq \rhomax$ then $\pp{\frac{\rhomax}{d}\I + \mH} $ is positive semidefinite. 
% \end{lemma}
% \begin{proof}
% \begin{align*}
%     \nn{\frac{\rhomax}{d}\I} = \rhomax
% \end{align*}

% First check that $\DET{\frac{\rhomax}{d}\I} = \pp{\frac{\rhomax}{d}}^d$

% Using the arithmetic/geometric mean inequality we have that $\DET{H} \leq \pp{\frac{\text{tr}(H)}{d}}^d$. Since $\text{tr}(H)\leq \nn{H}=\rhomax$ we have that 
% \begin{align*}
%     \DET{H} \leq \pp{\frac{\rhomax}{d}}^d
% \end{align*}
% Therefore $\DET{H}\leq \DET{\frac{\rhomax}{d}\I}$.
% \end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%
%% Begin exploration analysis
%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Exploration phase}


As usual let $T$ be the total number of episodes and in this section we 
let $\Texp \leq T$ be the number of episodes in the exploration phase. Let us define the regret in this phase as

\begin{align}
    \label{eq:regretExpI}
    R(\Texp) = \sum_{t=1}^{\Texp}\vdot{\thetabf^*, \va^*_t - \va_t}  
\end{align}
%


% We can easily bound the term 
Note that $\nn{\mH}\leq \sqrt{d}\rhomax$.
Initialize $\V_0 = 2\sqrt{d}\rhomax\I$. We let the exploration phase end when $\DET{\Vtil_t}\geq 2\DET{\V_0}$.
We need to bound the reward on each episode during the exploration phase.
On episode $t$, for any $\thetabf$ we have the following inequality:
{\color{blue} problem here. this is where epsilon shows up}
\begin{align}
    \notag
    \vdot{\thetabf - \thetahat_0, \va_t} 
    &= \vdot{\Vtil_t^{1/2}\pp{\thetabf - \thetahat_0}, \Vtil_t^{-1/2}\va_t}\\
    %%%
    \notag
    &\leq \nn{\Vtil_t^{1/2}\pp{\thetabf - \thetahat_0}}\nn{\Vtil_t^{-1/2} \va_t}\\
    %%%
    \notag
    &\leq \nn{\Vtil_t^{1/2}\pp{\thetabf - \thetahat_0}}
    \pp{\nn{\va_t}_{\Vtil_t^{-1}}}\\
    %%%
    \notag
    &\leq \sqrt{\frac{\DET{\Vtil_t}}{\DET{\Vtil_0}}}\nn{\Vtil_0^{1/2}\pp{\thetabf - \thetahat_0}}
    \pp{\nn{\va_t}_{\V_t^{-1}}}\\
     \notag
    &\leq \sqrt{2}\sqrt{2\sqrt{d}\rhomax}S
    \nn{\va_t}_{\V_t^{-1}}\\
    %%%
    % \notag
    % &\leq \sqrt{\rhomax} S\sqrt{2\nn{\va_t }^2_{\V_t^{-1}} } 
    % && \nn{\V}\leq \rhomax^2  \text{, } \nn{\thetabf^*}\leq S \\
    % %%%
    % \label{eq:regretExpII}
    % &\leq \sqrt{\rhomax} S\sqrt{2}\nn{\va_t }_{\V_t^{-1}} 
\end{align}
% the last inequality of \cref{eq:regretExpII} follows from $\va_t = \argmax_{\va\in\cA_t} \pp{1 + \nn{\va}_{\Vtil_t^{-1}}^2}$.


% For the next part, if $t\in U_{\Texp}$ we can use the trivial bound $\vdot{\thetabf^*, \va^*_t - \va_t}\leq 2$.
% Otherwise, if $t\not\in U_{\Texp}$ then by \cref{eq:regretExpII} we can use the following bound
% $\vdot{\thetabf^*, \va^*_t - \va_t}\leq \rhomax S\sqrt{2}\nn{\va_t }_{\Vtil_t^{-1}} \leq \rhomax S\sqrt{2\omega} $. The regret $R(\Texp)$ can be written as  
Now the regret in the exploration phase is given by
\begin{align*}
    \label{eq:regretExpIII}
    R(\Texp) &= \sum_{t=1}^{\Texp}\vdot{\thetabf^*, \va^*_t - \va_t} \\
    &\leq S\sqrt{2\sqrt{d}\rhomax} \sum_{t=1}^\Texp\nn{\va_t }_{\Vtil_t^{-1}} \\ 
    &\leq S\sqrt{2\Texp\sqrt{d}\rhomax} \sqrt{\sum_{t=1}^{\Texp}\nn{\va_t }^2_{\Vtil_t^{-1}}}  \\
    &\leq S\sqrt{2\Texp\sqrt{d}\rhomax} \sqrt{2\log\pp{\frac{\DET{\Vtil_\Texp}}{\DET{\Vtil_0}}}}  && \text{\cref{lem:elipticalPotential}} \\ 
     &\leq S\sqrt{2\Texp\sqrt{d}\rhomax} \sqrt{2\log\pp{2}}  && \text{\cref{lem:elipticalPotential}} \\ 
    &\approx O\pp{d^{1/4}\sqrt{\Texp / \eps}}
\end{align*}

% First we bound the second term of \cref{eq:regretExpIII}:
% \begin{align}\label{eq:regretExpIV}
%      \sum_{t\not\in U_{\Texp}}\vdot{\thetabf^*, \va^*_t - \va_t}
%      &\leq \sum_{t\not\in U_{\Texp}}\nn{\va_t }_{\Vtil_t^{-1}} \\
%      &\leq S\sqrt{2\rhomax} \sum_{t\not\in U_{\Texp}}\nn{\va_t }_{\Vtil_t^{-1}} \\ 
%      &\leq S\sqrt{2\rhomax} \sqrt{T}\sqrt{\sum_{t\not\in U_{\Texp}}\nn{\va_t }^2_{\Vtil_t^{-1}}}
% \end{align}


% Finally, letting $\omega = \frac{1}{\sqrt{T}}$ we get 
% \begin{align*}
%     R(\Texp) \leq \sqrt{\Texp} \pp{2\log\pp{\DET{\cE\I}} + 1} 
% \end{align*}




%%%%%%%%%%%%%%%%%%%%%%%%%
%% End exploration analysis
%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%
%% Begin: confidence sets
%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Confidence sets for $T\geq \Texp$}
\begin{lemma}
Let $\V_0 = \lambda\I$, define $r_t = \vdot{\va_t, \thetabf^*}$. For any $\delta>0$, with probability at least $1-\delta$, for all $t > \Texp$
\begin{align*}
    \nn{\thetahat_t - \thetabf^*}_{\V_t} \leq  \beta_t := R\sqrt{2\log\pp{\frac{\sqrt{\DET{\V_t}\DET{\lambda\I}}}{\delta}}}
    +\lambda^{1/2}S
\end{align*}
\end{lemma}

{\color{red}IDEA: Change regularizer when not in exploration phase.} 

Now we define the confidence set for  private counters
%
\begin{lemma}
Let $\Vtil_0 = 2\sqrt{d}\rhomax\I$, define $r_t = \vdot{\va_t, \thetabf^*}$.

 For any $\delta>0$, with probability at least $1-\delta$, for all $t > \Texp$
 \begin{align*}
 \nn{\thetahat_t - \thetabf^*}_{\Vtil_t} \leq   \beta_t := R\sqrt{2\log\pp{\frac{\sqrt{\DET{\Vtil_t}\DET{\frac{2\rhomax}{d}\I}}}{\delta}}}
    +S\sqrt{\frac{2\rhomax}{d}}
\end{align*}
\end{lemma}
%
\begin{proof}
Start with $\nn{\thetahat_t - \thetabf^*}_{\Vtil_t}  \leq  \nn{\Vtil_t^{1/2}\pp{\thetahat_t - \thetabf^*}}$.


Now we analyze $\nn{\Vtil_t}$. We showed that $\nn{\Vtil_t}\geq 2\rhomax$ for $t\geq \Texp$. Therefore $\nn{\V_t}\geq \rhomax$ and we have 
\begin{align*}
    \nn{\Vtil_t} = \nn{\V_t + \mH_t} \leq \nn{\V_t} + \nn{\mH_t} \leq 2\nn{\V_t}
\end{align*}
Therefore 
\begin{align}
% \label{eq:dpconfLemmaI}
    \nn{\thetahat_t - \thetabf^*}_{\Vtil_t}  &= 
    \nn{\Vtil_t^{1/2}\pp{\thetahat_t - \thetabf^*}}
    % \sqrt{\nn{\Vtil_t}} \nn{\thetahat_t - \thetabf^*} \\ 
    % &\leq \sqrt{2\nn{\V_t}} \nn{\thetahat_t - \thetabf^*}  \\
    % &\leq \sqrt{2} \nn{\thetahat_t - \thetabf^*}_{\V_t}  \\
\end{align}
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%
%% End: confidence sets
%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%
%% Begin: Exploration + Exploitation with optimism.
%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Exploration + Exploitation with optimism.}







\paragraph{Regret proof} Here we analyze the regret after the exploration phase.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Lemma
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{lem:regretI}
Consider $T > \Texp$.
For any $t>\Texp$, let 
$\V_t = \sum_{i=1}^t \va_t\va_t^\top + \V_0$, where $\V_0 = \frac{2\rhomax}{d}\I$
and $\Vtil_t = \V_t + \mH_t$ such that $\mH_t$ is the noise added by the binary mechanism.
Assume that for all $t$, $\nn{\mH_t}\leq \rhomax$ and we have $\nn{\thetabf_* - \thetahat_t}_{\Vtil_t^{-1}} \leq {\beta_t}$. Then the pseudo-regret of \cref{alg:lsb} is bounded by
\begin{align*}
    R(T) - R(\Texp) \leq \beta_T\sqrt{4  T \sum_{t=1}^T \min\bb{1, \nn{\avec_t}^2_{\Vtil_t^{-1}}}}
    \leq    \beta_T  \sqrt{4T 2d\log\pp{\frac{\mathrm{tr}\pp{\Vtil_1} + TL^2}{d\DET{\Vtil_1}^{1/d}}}}
    \approx O\pp{d^{1/4}\sqrt{T/\eps}}
\end{align*}
\end{lemma}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Lemma
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{lemma}\label{lem:regretII}
% % Let $\Vtil_t = \V_t + \mH_t$ such that $\mH_t$ is the noise added by the binary mechanism.
% Let $\va_1, \ldots, \va_T\in\bbR^d$ be vectors with $\|\va\|\leq L$. Given PSD matrix $\mU_1$, define $\mU_{t+1} = \mU_t + \va_t\va_t^\top$ for all $t$. Then
% %
% \begin{align*}
%     \sum_{t=1}^T \min\bb{1, \nn{\avec_t}^2_{\mU_t^{-1}}}\leq 2\log\pp{\frac{\det(U_{T+1})}{\det(U_1)}}
%     \leq 2d\log\pp{\frac{\text{tr}(U_1) + T L^2}{d(\det(U_1)^{1/d})}}
% \end{align*}
% \end{lemma}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Theorem
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{theorem}{(Regret)} With probability at least $1-\beta$ the regret of algorithm \cref{alg:lsb} is bounded by

% \begin{align*}
%     R(T) \leq \sqrt{4 (1+c) \beta_T T 2d\log\pp{\frac{\mathrm{tr}\pp{\Vtil_1} + TL^2}{d\DET{\Vtil_1}^{1/d}}}}
% \end{align*}
% \end{theorem}
% \begin{proof}
% Let $\va_1,\ldots, \va_T \in \pp{\cA_1\times,\ldots,\times\cA_T}$ be the sequence of actions by \cref{alg:lsb}. Let $\V_t = \sum_{i=1}^t \va_i\va_i^\top$ and $\y_t = \sum_{i=1}^t \va_t r_t$.
% %
% For all $t\in[T]$ we have that $\Vtil_t \leftarrow \cM_v(t)$ is an approximate count of $\V_t$ where $\cM:[T]\rightarrow \bbR^{d\times d}$ is a binary mechanism with privacy parameter $\eps$. Let us write $\Vtil_t = \V_t + \mH_t$ such that $\mH_t$ is the noise added by the binary mechanism.
% Likewise, let $\ytil_t = \y_t + \h_t$.

% With high probability we have that
% %
% \begin{align}\label{eq:regretI}
%     \rho_2 \I\succ \mH_t \succ \rho_1\I
% \end{align}
% It follows from \cref{eq:regretI}  that $\nn{\avec_t}^2_{\Vtil_t^{-1}}\leq \nn{\avec_t}^2_{\pp{\V_t^{-1} + \rho_1\I}}$. The confidence bound is given by
% \begin{align}
%     \sqrt{\beta_T} = 
% \end{align}


% %

% \begin{align*}
%     R(T) &\leq \sqrt{4 (1+c) \beta_T T \sum_{t=1}^T \min\bb{1, \nn{\avec_t}^2_{\Vtil_t^{-1}}}} \\ 
%     &\leq \sqrt{4 (1+c) \beta_T T \sum_{t=1}^T \min\bb{1, \nn{\avec_t}^2_{\pp{\V_t^{-1} + \rho_1\I}}}} && \text{\cref{eq:regretI}}\\
%     &\leq \sqrt{8 (1+c) \beta_T T 
%     d\log\pp{\frac{\text{tr}(\rho_1\I) + TL^2}{d\DET{\rho_1\I}^{1/d}}}} && \text{\cref{lem:regretII}}\\
%     &= \sqrt{8 (1+c) \beta_T T 
%     d\log\pp{\frac{d\rho_1 + TL^2}{d\rho_1}}} \\
%     &= \sqrt{8 (1+c) \beta_T T 
%     d\log\pp{1 + \frac{TL^2}{d\rho_1}}} \\
% \end{align*}

% \end{proof}



If we set $\V_1 = \Vtil_1 = \pp{\frac{\rhomax^2}{d} + \frac{\rhomax}{d}} \I$. then we have that for all $t>1$

\begin{align}
\Vtil_t = \V_t + \mH_t\succ \V_ \succ \frac{\rhomax^2}{d}\I  
\end{align}

%%%%%%%%%%%%%
%% Proof
%%%%%%%%%%%%%
\begin{proof}{(of \cref{lem:regretI})}
Let $r_t$ be the instantaneous regret at time $t$. 
Let $\tau$ be the last time step that the policy was updated. 

Then we can decompose the regret as:
\begin{align}\label{eq:LSBRegretDecomposition}
    r_t = \vdot{\theta_*, \va_*} - \vdot{\theta_*, \va_t} 
    \leq \vdot{\thetatil_{\tau}, \va_t} - \vdot{\theta_*, \va_t}  
    = \vdot{\thetahat_{\tau - 1} - \theta_*, \va_t}  + \vdot{\thetatil_{\tau } - \thetahat_{\tau-1}, \va_t}
\end{align}

Note that $\thetahat_{\tau - 1}$ is the center of the confidence set $C_{\tau - 1}$ and by definition of $C_{\tau-1}$ we have $\theta_*,\thetatil_{\tau} \in C_{\tau - 1} $ with high probability.

For any $\theta \in C_{\tau - 1}$ and $\x\in \bbR^d$ we have 
\begin{align*}
  \left| \vdot{\theta-\thetahat_{\tau-1}, \x} \right| &= \vdot{\Vtil_t^{1/2}(\theta-\thetahat_{\tau-1}), \Vtil_{t}^{-1/2} \x}  \\ 
    &\leq \nn{\Vtil_t^{1/2}(\theta-\thetahat_{\tau-1}) } \sqrt{\x^\top \Vtil_t^{-1} \x}  \\ 
    &\leq \nn{\Vtil_{\tau-1}^{1/2}(\theta-\thetahat_{\tau-1}) } 
            \sqrt{\frac{\det\pp{\Vtil_t}}{\det\pp{\Vtil_{\tau-1}}}}
            \sqrt{\x^\top \Vtil_t^{-1} \x}  \\ 
    &= \nn{\theta-\thetahat_{\tau-1} }_{\Vtil_{\tau-1}}
            \sqrt{\frac{\det\pp{\Vtil_t}}{\det\pp{\Vtil_{\tau-1}}}}
            \sqrt{\x^\top \Vtil_t^{-1} \x}  \\ 
    &\leq \sqrt{(1+c)\beta_{\tau-1}}\sqrt{\x^\top \Vtil_t^{-1}\x}
  = \sqrt{(1+c)\beta_{\tau-1}}\nn{ \x}_{\Vtil_t^{-1}} 
\end{align*}


Since $r_t\leq 2$, we can write \cref{eq:LSBRegretDecomposition} as 
\begin{align}\label{eq:LSBRegretDecomposition}
    r_t &\leq 2 \min\pp{ \sqrt{(1+c)\beta_{\tau-1}}\nn{ \va_t}_{\Vtil_t^{-1}}, 1} \\ 
    &\leq 2 \sqrt{(1+c)\beta_{\tau-1}}\min\pp{\nn{ \va_t}_{\Vtil_t^{-1}} , 1}
\end{align}


Using Cauchy-Schwartz inequality we have with probability $1-\beta$:
\begin{align*}
    R(T)  &= \sum_{t=1}^T r_t \leq \sqrt{T \sum_{t=1}^T r_t^2} \\
    &\leq \sqrt{4T(1+c)\beta_{T} \sum_{t=1}^T \min(\nn{ \va_t}^2_{\Vtil_t^{-1}}, 1) } \\ 
    &\leq \sqrt{8T(1+c) \beta_T  \log\pp{\frac{\det(\Vtil_T)}{\det(\Vtil_0)}}}
\end{align*}
\end{proof}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% endgroup
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endgroup

==> files/old/slow_update_lemma.tex <==
\section{Slow Update Lemma}



%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Lemma: Bounding updates
%% Make Lemma general enough that it can be applied to the linear bandits setting.
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{lem:Switchingcost}
Let $\phibf_1, \ldots, \phibf_T$ be a  sequence  of length $T$, where each $\phibf_t\in\bbR^d$ is a $d$-dimensional vector and for all $t\in[T]$ it holds that $\nn{\phibf_t}_2\leq 1$. 
For each $t\in[T]$, define $\W_t = \sum_{i=1}^{t} \phibf_i \phibf_i^\top + \V$
where  $\V\in \bbR^{d\times d}$  is any positive semidefinite matrix. 
Let $c>1$ be any constant and say that there is a trigger event on time $t$ if $\det\pp{\W_t} \geq c \det\pp{\W_{\tau}}$, where $\tau<t$ is the time of the last trigger event before $t$ or 0 if $t$ is the first trigger event.

If there exists $\lambda>0$ such that $\mathrm{tr}(\V) \leq  d\lambda$, $\det\pp{\V} \geq \lambda^d$ and $d\lambda \geq \frac{T}{T-1} $, then the number of trigger events is at most $d  \LOG{c}{T}$.
\end{lemma}

\begin{remark}
We can satisfy the assumption in \cref{lem:Switchingcost} by setting $\V = \lambda \I$. 
Note that to set the right value of $\lambda$ we must know $T$ in advance.
\end{remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
\newcommand{\ki}[1]{k_{[#1]}}


Let $K$ be the total number of trigger events at the end of  $T$ rounds and let $\ki{0}, \ldots, \ki{K}$ be the trigger event times. By definition the first and last rounds are trigger events, thus we have $\ki{K} = T$  and $\ki{0} = 0$. We proceed by assuming that $K > d\LOG{c}{T}$ and show that this leads to a contradiction.

First, by definition of a trigger event on time $\ki{K}$ we have 
%
\begin{align}\label{eq:mainI}
    c \DET{\W_{\ki{K-1}}} \leq \DET{\W_{\ki{K}}}
\end{align}

If we unfold the recursion given by \cref{eq:mainI} and starting with $c \DET{\W_{\ki{K-1}}} $ we get the following inequality
\begin{align}\label{eq:inductiveinequalityI}
    c\DET{\W_{\ki{K-1}}}
    \geq c^2 \DET{\W_{\ki{K-2}}}
    \geq c^3 \DET{\W_{\ki{K-3}}}
    \geq \ldots 
    \geq c^{K} \DET{\W_{\ki{0}} }
\end{align}

Note that $c^{d\LOG{c}{\ki{K}}}  = c^{\LOG{c}{\ki{K}^d}}  = \ki{K}^{d}$.
Since $c>1$ and by the assumption that $K > d\LOG{c}{\ki{K}}$, the following holds $c^{K} > c^{d\LOG{c}{\ki{K}}}=\ki{K}^{d}$. Therefore, combining \cref{eq:mainI} and \cref{eq:inductiveinequalityI} and replacing $K$ with $ d\LOG{c}{\ki{K}}$ we have
%
\begin{align}
\label{eq:mainII}
    \text{\cref{eq:mainI}, \cref{eq:inductiveinequalityI}} \text{ and } K > d\LOG{c}{\ki{K}}
    \implies \ki{K}^{d} \DET{\W_{\ki{0}} } < \DET{\W_{\ki{K}}} 
\end{align}
%
Next, we use the fact that the determinant a matrix is equal to the product of its eigenvalues and the trace of a matrix equals the sum of its eigenvalues and we use the  inequality of arithmetic and geometric means to get
%
\begin{align}\label{eq:AGmeans}
    \DET{\W_{\ki{K}}} \leq \pp{\frac{\text{tr}\pp{\W_{\ki{K}}}}{d}}^d 
    % \label{eq:clogD}
    % c^{d\LOG{c}{\ki{K}}}  = c^{\LOG{c}{\ki{K}^d}}  = \ki{K}^{d}
\end{align}

Combining \cref{eq:mainII}, \cref{eq:AGmeans} we get
%
\begin{align} \label{eq:mainIII}
    \text{\cref{eq:mainII}, \cref{eq:AGmeans}} \implies 
    \ki{K}^{d}\DET{\W_{\ki{0}} } < \pp{\frac{\text{tr}\pp{\W_{\ki{K}}}}{d}}^d
\end{align}

For the next step, we use the  fact that $\text{tr}\pp{\W_{\ki{K}}} \leq \text{tr}\pp{\W_{0}} + \ki{K} $, which follows from the assumption that $\nn{\phibf_i}_2^2 \leq 1$. Then it follow from \cref{eq:mainIII} that

\begin{align} \label{eq:mainIV}
    \text{\cref{eq:mainIII}} \implies 
    \ki{K}^{d}\DET{\W_{\ki{0}} } < \pp{\frac{\text{tr}\pp{\W_{\ki{0}}}  + \ki{K}}{d}}^d
\end{align}

Dividing $\ki{K}$ on both sides of equation \cref{eq:mainIV} we get
\begin{align} \label{eq:mainV}
    \DET{\W_{\ki{0}} } 
    <  \pp{\frac{\text{tr}\pp{\W_{\ki{0}}}  + \ki{K}}{d \ki{K}}}^d  
    = 
    \pp{\frac{\text{tr}\pp{\W_{\ki{0}}}}{d \ki{K}} 
    + \frac{1}{d}
    }^d
\end{align}

We assumed that $\DET{\W_{\ki{0}}} \geq \lambda^d$ and that $\text{tr}\pp{\W_{\ki{0}}} \leq d\lambda$, thus \cref{eq:mainV} implies
\begin{align} 
\notag
\text{\cref{eq:mainV}} &\implies 
    \lambda^d < \pp{\frac{d\lambda}{d \ki{K}} + \frac{1}{d} }^d  \\
    \label{eq:mainVI}
    &\implies
    1 <  \pp{\frac{d\lambda}{d \lambda\ki{K}} + \frac{1}{d\lambda} }^d 
    =  \pp{\frac{1}{\ki{K}} + \frac{1}{d\lambda} }^d 
    = \pp{\frac{1}{T} + \frac{1}{d\lambda} }^d 
\end{align}

Since we choose $d\lambda $ s.t $\frac{1}{T} + \frac{1}{d\lambda} \leq 1$ then \cref{eq:mainVI} is a contradiction completing the proof.
\end{proof}


% \begin{proof}
% \newcommand{\ki}[1]{k_{[#1]}}
% % Fix time-step $h$. Let $\phibf_t = \phi\pp{x\ii{t}{h},a\ii{t}{h}}$ be the observed feature vector on time $(t,h)$ for all $t\in[T]$.
% % We use $\W_t = \Lambtil_h^t$ to denote the gram matrix on $(t,h)$.
% % Let $\V$ be a positive semi-definite matrix with minimum eigenvalue $\lambda_0 = \lambda_{min} (V)$. Then we can write $\W_t$ as
% % \begin{align*}
% % \W_t = \sum_{i=1}^{t-1} \phibf_i \phibf_i^\top + \V
% % \end{align*}
% We use an inductive argument to show that trigger events are sufficiently spread out.
% Let $\{i\}_{i=1}$
% Let $\ki{i} \in [T]$ denote the time step of the $i$-th trigger event, where $\ki{0} = 1$. Our goal is to show that for all $i>0$, we have $\ki{i} > D \ki{i-1}$, which would imply that there are at most $\log_D(T)$ trigger events.

% We prove this by induction:

% \paragraph{Base case} First, we show that $k[1] > D \ki{0} = D$.
% {\color{red} gv: Add proof here. } \\

% \paragraph{Inductive step:} Fix $i>1$ and assume that for all $j < i$ we have $\ki{j} \geq D \ki{j-1}$. This assumption says that up to time step $\ki{j}$ the has been at most $\log_D\pp{\ki{j}}$ trigger events, for all $0 < j < i$. The assumption also implies that for all $j$ such that $j<i$ we have $j \leq \LOG{D}{\ki{j}}$, since the index $j$ represents the $j$-th trigger event.

% To complete the argument, we have to show that $\ki{i} \geq D \ki{i-1}$. We assume that $\ki{i} < D \ki{i-1}$ and show that this leads to a contradiction. Recall that $c$ is the trigger ratio, 
% thus be definition of a trigger event on time $\ki{i}$ we have the following inequality, 

% \begin{align}\label{eq:cdetrec}
%     c \DET{\W_{\ki{i-1}}} \leq \DET{\W_{\ki{i}}}
% \end{align}
% %
% If we unfold the recursion given by \cref{eq:cdetrec} and starting with $c \DET{\W_{\ki{i-1}}} $ we get the following equation:
% \begin{align}\label{eq:inductiveinequalityI}
%     \DET{\W_{\ki{i-1}}}
%     \geq c \DET{\W_{\ki{i-2}}}
%     \geq c^2 \DET{\W_{\ki{i-3}}}
%     \geq \ldots 
%     \geq c^{i-1} \DET{\W_{\ki{0}} }
% \end{align}

% %
% By the inductive assumption, on time $\ki{i-1}$ there are at most $\LOG{D}{\ki{i-1}}$ trigger events, that means that $i-1\leq \LOG{D}{\ki{i-1}}$. Then we can we obtain a lower bound for $c \DET{\W_{\ki{i-1}}}$, using \cref{eq:inductiveinequalityI} and replacing $i-1$ by $\LOG{D}{\ki{i-1}}$ as follows,
% \begin{align}
%      c \DET{\W_{\ki{i-1}}}  \geq  c^{1 + \LOG{D}{\ki{i-1}} } \DET{\W_{\ki{0}} }
% \end{align}
% % \begin{align}\label{eq:inductiveinequality}
% %     c \det\pp{\W_{\ki{i-1}}}
% %     \geq c^2 \det\pp{\W_{\ki{i-2}}}
% %     \geq \ldots 
% %     \geq c^{\LOG{D}{\ki{i-1}}} \det\pp{\W_{\ki{1}} }
% % \end{align}

% Next, we use the fact that the determinant a matrix is equal to the product of its eigenvalues and the trace of a matrix equals the sum of its eigenvalues and we use 
% the  inequality of arithmetic and geometric means to get
% %
% \begin{align}\label{eq:AGmeans}
%     \DET{\W_{\ki{i}}} \leq \pp{\frac{\text{tr}\pp{\W_{\ki{i}}}}{d}}^d
% \end{align}

% combining \cref{eq:cdetrec}, \cref{eq:inductiveinequality} and \cref{eq:AGmeans} we have
% %
% \begin{align}\label{eq:cdetI}
%     c^{\LOG{D}{\ki{i-1}}} \DET{\W_{1}} \leq \DET{\W_{\ki{i}}} \leq \pp{\frac{\text{tr}\pp{\W_{\ki{i}}}}{d}}^d
% \end{align}

% For the next step, we use the following fact $\text{tr}\pp{\W_{\ki{i}}} \leq \text{tr}\pp{\W_{1}} + \ki{i} $, which follows from the assumption that $\nn{\phibf_i}_2 \leq 1$ and the assumption that $\ki{i} < D \ki{i-1} = 2^{1/d} \ki{i-1}$. 
% %
% \begin{align}\label{eq:cdetII}
%     c^{\LOG{D}{\ki{i-1}}} \DET{\W_{1}} 
%     % \leq \pp{\frac{\text{tr}\pp{\W_{1}} + \ki{i}}{d}}^d 
%   <   \pp{\frac{\text{tr}\pp{\W_{1}} + D \ki{i-1}}{d}}^d
% \end{align}



% Let $D = c^{1/d}$, then
% \begin{align}\label{eq:clogD}
%     c^{\LOG{D}{\ki{i-1}}} 
%     = c^{\frac{\LOG{c}{\ki{i-1}}}{\LOG{c}{D}}}
%     = \pp{\ki{i-1}}^{\frac{1}{\LOG{c}{c^{1/d}}}}
%     = \pp{\ki{i-1}}^{d}
% \end{align}

% % {\color{red} gv:This next assuption is not right. we need to } \\
% Note that $\W_1 = V$ and
% recall that $\det(\W_1) > \lambda_0^d$ and $\text{tr}(\W_1) < d\lambda_0$. Then, \cref{eq:clogD} and \cref{eq:cdetII} implies
% %
% \begin{align}\label{eq:eq:cdetIII}
%     \ki{i-1}^d \lambda_0^d  < \pp{\frac{d\lambda_0 + c^{1/d} \ki{i-1}}{d}}^d 
% \end{align}




% This implies 
% %
% \begin{align*}
%     1  & <   \frac{ d\lambda_0+ c^{1/d} \ki{i-1}}{d\lambda_0 \ki{i-1}} \\ 
%     &= \frac{1}{ \ki{i-1}} + \frac{c^{1/d}}{d\lambda_0}
% \end{align*}

% Since $i>2$ we have that $\ki{i-1} \geq 2$ and also by assumption 
% $d \geq 2$ 
% \end{proof}


==> files/outline.tex <==
\section{Outline}
\begin{enumerate}
    \item \textbf{Introduction}:
         \begin{enumerate}
             \item Describe differential privayy in the batch setting and then in the online setting.
             \item Why is differential privacy in RL is important and mention previous work in this area: DP in the tabular RL setting \cite{vietri2020private}, DP in the linear bandits setting \cite{sheffet2017differentially}, local DP in the tabular setting \cite{garcelon2020local}
             
      
             \item In the tabular setting, the best non-private algorithm has regret that grown with $O(\sqrt{K})$, \cite{dann2019policy}, where $K$ is the number of episodes.
             
             \item Also in the tabular setting, \cite{vietri2020private} provides a model-based algorithm based on \cite{dann2019policy} that satisfies global differential privacy and has a regret term that is proportional to $O(\sqrt{K})$ and has an additional term that grows with $O( \frac{\log(K)}{\epsilon} )$, where $\epsilon$ is the privacy parameter.
             Therefore, in the tabular setting the result from \cite{vietri2020private}, shows  that when the number of episodes is large the cost of privacy is lower order in $K$. 
             \item In this paper we study the linear MDP setting, where the state space of the environment is to large to count. In this setting, we use the assumption that the environment is determined by a linear function of the states and actions.  The linear MDP setting can model more realistic scenarios 
             \item The most recent paper to study the linear MDP setting with privacy is \cite{luyo2021differentially}, which gives a model free algorithm with suboptimal additional privacy regret with a polynomial dependence on $K $(the number of episodes). 
             \item Therefore the  key Question is: Can we get $\log(K)$ dependence on the private regret in the linear MDP setting? 
             \item Explain why \cite{luyo2021differentially}, couldn't obtain the $\log(K)$ regret rate. Answer: They updated the policy using fixed interval epsisodes in a data-independent way.
             
             \item Why can't we use the binary mechanism in the linear MDP setting?
             \item Our contribution is to update the policy in a data-dependent way such that we do at most $d\log(K)$ policy updates and show that the algorithm still satisfies global differential privacy. 
             \item Cite the privacy filter paper \cite{lecuyer2021practical} as our main tool to analyze the privacy 
             \item This approach recovers the desired $\log(K)$ regret bound.
         \end{enumerate}
    \item Prelims
    \item Related work
    \item \textbf{Explain the algorithm}:
    \begin{enumerate}
        \item 
    \end{enumerate}
    \item \textbf{Privacy Analysis}:
    \begin{enumerate}
        \item Show how to analyze data depended updates using a privacy filer. First we demonstrate that the interaction in \cref{alg:privrl} is equivalent to the adversary in the privacy filter paper.
    \end{enumerate}
    \item \textbf{Regret Analysis}
\end{enumerate}

==> files/theorems/jdp/proof.tex <==
\begin{proof}



\cref{alg:privrl} uses two zCDP mechanisms (the Binary Mechanism and the Adaptive Gaussian mechanism.) that each satisfy $(\rho/2)$-zCDP, such that the composition of the two satisfies $\rho$-zCDP. Then by composition the algorithm satisfies $\rho$-zCDP. 




The Binary mechanism \cite{shariff2018differentially}, which keeps track of the noisy covariance matrix $\Lambtil_k$, privacy guarantee is given by \cref{lem:}. The main analysis in this section is the analysis of the adaptive Gaussian mechanism.


The adaptive Gaussian mechanism releases a vector $\ytil_k$ every time there is an update episode in \cref{alg:privrl}.

\paragraph{Adaptive Gaussian Analysis} First, we describe the interaction between an adversary and the algorithm. Fix a bit $b \in \{ 0, 1 \}$.
Suppose that during each episode $k$ of the algorithm, an adversary observes the events $\ytil_1, \ldots, \ytil_{k-1}$ and based on that it chooses two neighboring datasets $D^0_k$ and $D^1_k$ and a function $f_k$.
If \cref{lin:update} in \cref{alg:privrl} is true then the adversary chooses $f_k(D_k^{b}) = \sum_{i=1}^{k-1}\phib{x\ii{i }{h}, a\ii{i}{h}} \left( r_h(x\ii{i }{h}, a\ii{i}{h}) +\max_{a\in\cA}Q_{h+1}^{\tau_h}(x_{h+1}^i, a) \right)$.
Otherwise, the adversary chooses $f_k$ to by a constant function that always outputs the zero vector \footnote{Note that the constant function is not  part of \cref{alg:privrl} and it's only used for this analysis. }.
%

Then, by \cref{lem:sensitivity} and \cref{thm:switchingcost} we have that 
\begin{align*}
        \sum_{k=1}^K \|f_k(D_k^0) - f_k(D_k^1) \|_2 \leq (2H +2) d H \log(K):=\Delta
\end{align*}


Next we define a class of $\left(\frac{\rho}{\Delta}\right)$-zCDP Gaussian mechanisms as follows:
For any $k\in [K]$, let $\cM_k(D_k^b) = f_k(D_k^b) + \eta_k$, where $\eta_k \sim \cN(0, \frac{\Delta}{\rho})$.


% be the Gaussian mechanism that approximates  the value of $f_k$ such that it satisfies $\left(\frac{\rho}{\Delta}\right)$-zCDP. That is $\cM_k(D_k^b) = f(D_k^b) + \eta_k$.
%
The final step is the interaction with the adversary is that it observes a realized output $\ytil_k \sim \mathcal{M}_k(D_k^b)$.



%
% If a policy update happens in episode $k$, the adversary observes a realized output $v_k \sim \mathcal{M}_k(D_k^b)$. Else, the adversary observes a constant function $v_k = (0, \dots, 0)$. 
Then, by \cref{lem:gaussianadaptivecomp} the outputs $\ytil_1, \ldots, \ytil_K$ of this interaction satisfy $\rho$-zCDP. 

\end{proof}


==> files/theorems/swtichingcost_gao/proof.tex <==
\newline
Combining the lemmas above, we can now prove the switching cost bound in \Cref{thm:switchingcost}
\begin{proof}
Let $\{ k_1, k_2, \dots, k_{N_\text{switch}^\text{gl}} \}$ denote the update episodes $\tilde{k}$ from \Cref{alg:privrl}. By 
\Cref{lem:L2-switchingcost} we know $\det \Lambtil_{k_{i+1}} \geq 2 \det \Lambtil_{k_i} \geq 2^{k_{i+1}}\det \Lambtil_0$. Hence, by combining \Cref{lem:potentialupperGao} we have $N_{\max} \geq c_0 \log \det \Lambtil_K = O(d \log K)$
\end{proof}


==> files/todo.tex <==
\section{TODO}:
last updated Jan 21.

